Equal Bits: Enforcing Equally Distributed Binary Network Weights

Binary networks are extremely efficient as they use only two symbols to define the network: $\{+1,-1\}$. One can make the prior distribution of these symbols a design choice. The recent IR-Net of Qin et al. argues that imposing a Bernoulli distribution with equal priors (equal bit ratios) over the binary weights leads to maximum entropy and thus minimizes information loss. However, prior work cannot precisely control the binary weight distribution during training, and therefore cannot guarantee maximum entropy. Here, we show that quantizing using optimal transport can guarantee any bit ratio, including equal ratios. We investigate experimentally that equal bit ratios are indeed preferable and show that our method leads to optimization benefits. We show that our quantization method is effective when compared to state-of-the-art binarization methods, even when using binary weight pruning.

==> bkp_experiments_new_bkp.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{c@{\hskip 1in}c}
    \includegraphics[width=0.44\textwidth]{fig/eweight_hitting/flipped_uneven.png} & \\   
    \small {(a) $Sign$ has uneven flips by independently updating binary weight.} & \\
    \includegraphics[width=0.44\textwidth]{fig/eweight_hitting/IRnet_flipped_even.png} & \\ 
    \small {(b) IR-Net has uneven flips by balancing the latent weights.} &  \\
    \includegraphics[width=0.46\textwidth]{fig/eweight_hitting/bihalf_flipped_even.png} & \\
    \small {(c) \Model has even flips by precisely controlling the flipping. } & \\ 
    \end{tabular}
    \caption{\small \textbf{Exp 1: Bit flip during training.}
    We compare the bit flips during training in our \model with the $sign$~\cite{rastegari2016xnor} and IR-Net~\cite{qin2020forward} on the Conv2 network. 
    In contrast to $sign$ and IR-Net, our \model method achieves the ideal equal bit distribution.
    }
    \label{fig:envenflip}
\end{figure}

%---------------------------------------------------------------------------------------
\section{Experiments}
\noindent \textbf{Datasets and implementation details.} 
We evaluate on Cifar-10, Cifar-100~\cite{krizhevsky2009learning} and ImageNet~\cite{deng2009imagenet}, for number of network architectures.
Following~\cite{frankle2018lottery,ramanujan2020s} we evaluate 4 shallow CNNs: Conv2, Conv4, Conv6, and Conv8 with 2/4/6/8 convolutional layers.
We train the shallow models on Cifar-10 for 100 epochs, with weight decay $1e^{-4}$, momentum 0.9, batch size 128, and initial learning rate 0.1 using a cosine learning rate decay~\cite{loshchilov2016sgdr}.
Following~\cite{qin2020forward} we also evaluate their ResNet-20 architecture and settings on Cifar-10.
On Cifar-100, we evaluate our method on 5 different models described below. 
We train the Cifar-100 models for 350 epochs using SGD with weight decay $5e^{-4}$, momentum 0.9, batch size 128, and initial learning rate 0.1 divided by 10 at epochs 150, 250 and 320.
For ImageNet we use ResNet-18 and ResNet-34 trained using SGD with momentum $0.9$, weight decay $1e^{-4}$, and batch size 256.
All our models are trained from scratch without any pre-training.
For the shallow networks we apply our method on all layers, while for the rest we follow~\cite{liu2018bi,qin2020forward}, and apply it on all convolutional and fully-connected layers except the first, last and the downsampling layers. 
We share all code\footnote{Link to our github source code omitted for review}.

%---------------------------------------------------------------------------------------



% \begin{figure*}[t]
%     \centering
    
%         \begin{tabular}{c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
%     \includegraphics[width=0.48\textwidth]{fig/eweight_hitting/weight_gradhitting.png} &\ \ \ \  \ \ \
%         \includegraphics[width=0.48\textwidth]{fig/eweight_hitting/flipped_uneven.png} & \ \ 
%     % \slp{Is this IR-NET? We should compare with IR-NEt for exp 1.} 
%     \\   
%     \small {(a) How is a single binary weight flipped. }  & \ \ \ \ \ \ \
%     \small {(b)
%     % Sign independently flips the binary weights within a  filter.
%      Sign   has  uneven flips by independently updating binary weight.  
%     % within binary weight filter
%         % Sign: how are the binary weights flipped within a  filter.
%         } & \\
%             \includegraphics[width=0.48\textwidth]{fig/eweight_hitting/IRnet_flipped_even.png} & \ \ \ \  \ \ \
%     % \slp{Is this IR-NET? We should compare with IR-NEt for exp 1.} \\  
%         \includegraphics[width=0.48\textwidth]{fig/eweight_hitting/bihalf_flipped_even.png}
%  \\ 
%   \small {(c) IRnet   has  uneven  flips by   balancing latent weights.
% %   how are the binary weights flipped within a  filter.  
%   } & \ \ \ \ \ \ \
%   \small {(d) Bihalf has  even flips by  precisely controlling the flipping. }  \\ 
%                 \end{tabular}
%     \caption{\small
%     Flips of binary weights during training. The (a) shows how a single binary weight flips by comparing the gradient with the latent weight. 
%     The (b, c, d)  compares the flipped number within a filter between our Bihalf method and two other methods, Sign and IRnet.  
%     In each subfigure, the left one plots the flips of (+1 to -1) and (-1 to +1) for a single iteration, and the right one shows the total flips as training.  
%     We find that the Sign and IRnet have uneven flips during training which is hard to control the binary weight distribution.   
% Our proposed bihalf method has even flips by precisely controlling the binary weight distribution. 
%     % \slp{This plot is nice for exp 1.}
%     }
%     \label{fig:envenflip}
% \end{figure*}




\begin{figure*}[t]
    \centering
    \begin{tabular}{c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
            \includegraphics[width=0.198\textwidth]{fig/Flipping_Decayeffect/Mean_weight_vsweidecay.pdf} & \  
            \includegraphics[width=0.1928\textwidth]{fig/Flipping_Decayeffect/gradmagiter_vslearningrate.png}   & \ 
         \includegraphics[width=0.196\textwidth]{fig/Flipping_Decayeffect/Flippednumber_vsweidecay.pdf} &  \  
                                  \includegraphics[width=0.196\textwidth]{fig/Flipping_Decayeffect/Flippednumber_vslearningrate.pdf} &   \ 
    \includegraphics[width=0.194\textwidth]{fig/Flipping_Decayeffect/ACC_weigthdecay_lr.pdf}  \\
   \ \ \   \ \ \  \small (a) weights decay & \ 
  \ \ \   \small (b)  learning rate schedule & \     
  \ \ \   \small (c)  flips with cosine Lr& \ 
  \ \ \   \small (c)  flips with constant Lr& \ 
   \ \ \ \   \small (e) accuracy  & \     
    %  \multicolumn{2}{c}{\ \ \ \ \ \ \ \ \ \  TTQ} \\
    %  \ \ \ \ \ Conv4 &  \ \ \ \ Conv8  \\
    \end{tabular}
    \caption{\small
    Effect of different training techniques on binary weights flips. 
    % \textbf{Exp 2: Comparison with ternary strategies.}
    % Ternary weights distribution over the epochs on Cifar-10 using Conv4/6/8.
    % For  TWN method,  the distribution of $+1$ and $-1$ is not well balanced. 
    % TTQ induces lower sparsity as the network gets deeper. 
    % We utilize optimal transport to precisely control the weight distribution throughout the whole training process.
    }
     \label{fig:TTQ_epochs}
\end{figure*}

% \begin{figure*}[t]
%     \centering
    
%         \begin{tabular}{c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
%     \includegraphics[width=0.47\textwidth]{fig/eweight_hitting/weight_gradhitting.png}
%     \small {(a) Flipping by comparing dynamic threshold with gradient}  
%         \includegraphics[width=0.47\textwidth]{fig/eweight_hitting/flipped_uneven.png} &
%     \small {(b)  Sign  has  unevenly  flipping within binary weight filter} 
%     % \slp{Is this IR-NET? We should compare with IR-NEt for exp 1.} 
%     \\   
%             \includegraphics[width=0.47\textwidth]{fig/eweight_hitting/IRnet_flipped_even.png}\\
%     \small {(c) IRnet  has  unevenly  flipping within binary weight filter}  \\
%     % \slp{Is this IR-NET? We should compare with IR-NEt for exp 1.} \\ 
%         \includegraphics[width=0.47\textwidth]{fig/eweight_hitting/bihalf_flipped_even.png}
%             \small {(d) Bi-half    has  evenly  flipping within binary weight filter.}  \\ 
%                 \end{tabular}
%     \caption{\small
%     Binary weight flips during training. (a) single binary weight flip; (b, c):  binary weight flips within a filter
%     % \slp{This plot is nice for exp 1.}
%     }
%     \label{fig:envenflip}
% \end{figure*}



% \begin{figure}[t]
%     \centering
%     \begin{tabular}{c@{}c@{}c@{}}
%       \multicolumn{3}{c}{\includegraphics[width=0.23\textwidth]{fig/exp1/Legend_sign.pdf}} \\
%     \includegraphics[width=0.175\textwidth]{fig/exp1/Sign_percentage_onefilter_conv2_layer.pdf} &\ 
%     \includegraphics[width=0.145\textwidth]{fig/exp1/IR_net_percentage_filter_conv2_layer.pdf} & \ 
%     \includegraphics[width=0.145\textwidth]{fig/exp1/ours_bihalf_conv2.pdf} \\
%      \ \ \ \ \  \ \ Sign &  \ \ \ \ {IR-net} & \ \ \ \ Ours  \\
%     \end{tabular}
%     \caption{\small
%     % \textbf{Exp 2.1: Comparison with other strategies using Conv4.}
%     Binary 
% weights distribution for different methods  over the epochs on Cifar-10 using Conv2.
%     % Ternary weights distribution over the epochs on Cifar-10 using Conv2.
%     % For TWN we observe that as training proceeds, the sparsity gets higher $\sim$60\%, and the positive and negative percentages reduce to $\sim$15\% and $\sim$25\%; where the distribution of $+1$ and $-1$ is not well balanced.
%     % TTQ introduces trainable scaling coefficients to help balancing the distribution of $-1$ and $+1$, and it achieves a $\sim$20\% sparsity, and $\sim$40\% of positives and negatives.
%     % We utilize optimal transport to precisely control the weight distribution throughout the whole training process.
%     }
%      \label{fig:TTQ_epochs}
% \end{figure}


\begin{comment}
\subsection{Effect of training techniques
}
We study some commonly
used techniques such as  weight clipping, regularization and learning rate decay, and show that some of these techniques are not crucial in training well-performing BNNs.
% We further study the effectiveness of the various commonly  used  training  techniques.
\begin{itemize}
\item $L_2$ regularization. We find that applying L2-regularization to the real-valued threshold  should not lead to any regularization. It only  affects binary weight flips by controlling the magnitude of threshold as shown in \fig{envenflip}(a). 
\item Bipolar regularization.
Some recent works \yq{citation}
%How to Train a Compact Bnn, 1-Bit CNNs, Rotated Binary Neural Network, BNN++
introduce regularization term or design specific loss function to encourage real-valued parameter to  binary weight. We show that encouraging  real-valued threshold to be bipolar distribution is not necessary. 
\item Weight clipping. 
Clipping is used to restrict the latent weights as in common view between a region that avoids latent weights grow very large. We reveal that clipping of the threshold is not crucial during training. 
% \item Scaling factors. 
% add a real-valued scaling factor to imporve the 
\item Learning rate decay.  
Bop claims that scaling of the learning rate does not affect training.  
We find that varying  learning rate as  in \eq{behalf} will affect binary weight flips.
Gradually reducing learning rate will decrease weight flips. 
We also find that the learning rate decay and the $L_2$ regularization are indispensable to each other.
% This variable $\alpha$ should 
% As in real-valued network, learning rate is used to control the updated step size 
\end{itemize}
Our interpretation of latent weights as dynamic threshold is easy to reason about the effectiveness of various optimization techniques.  
We will further explore their effectiveness  in the experiments section. 
\end{comment}

%------------------------------------------------------------------------------------------
\subsection{\textbf{Exp 1}: Bi-half maximizes the entropy} 
In \fig{envenflip} we compare the proposed  optimization method  Bihalf to the two existing methods, Sign~\cite{rastegari2016xnor} and IRnet \cite{qin2020forward}. We train a Conv2 network on Cifar10  and  plot the flips of binary weights in a single binary weight filter as training.  The binary weights are initialized to be half-half distributed at beginning. 

For each row,  the x-axis shows the training iterations; the y-axis in left sub-figure shows the flips per training iteration and the y-axis in right sub-figure denotes the total flips for all previous training iterations.  
    (a) Classical Sign method~\cite{rastegari2016xnor}  binarizes each weight independent of the other weights. During training the flips for (+1 to -1) and  (-1 to +1) are uneven. 
    (b) IRnet~\cite{qin2020forward} balances the latent weights with their statistics to obtain evenly distributed binary weight values. It can not guarantee the binary weights to be evenly distributed. 
    (c) Bihalf updates the binary weight depending on the statistics of the other weights.  
    Per iteration, the binary weights are evenly flipped. 

          The classical binarization method in  \fig{envenflip}(a) quantizes each weight independent of the other weights making the binary weights unevenly distributed. Rather than updating the weights independent of each other, IRnet in  \fig{envenflip}(b)
          uses weight statistics for updating the binary weights. This work will get fail when the latent weights are not symmetric distributed.  
          The proposed  Bihalf method in  \fig{envenflip}(c) updates the binary weight depending on the statistics of the other weights.  During training, the binary weights are controlled to be evenly flipped. 
    It can achieve the ideal half-half distribution.

In \fig{entropybitratio}
%-------------------------------------------------------------------------------------------------
\subsection{\textbf{Exp 2:} Empirical analysis of bi-half   approach}

\begin{figure}[t]
\centering
\begin{tabular}{cc}
    {(a) Full binary network} &
    {(b) \Model network} \\
    \includegraphics[width=0.22\textwidth]{fig/toy/AAAISign_figure_sign1.pdf} &
    \includegraphics[width=0.22\textwidth]{fig/toy/AAAISign_figure_half_half1.pdf} \\
    \scriptsize{Weight combinations: 4096.} &
    \scriptsize{Weight combinations: 924.} \\
    \scriptsize{Unique solutions: 76.} &
    \scriptsize{Unique solutions: 66.} \\
    \end{tabular}
    \caption{ \small
    \textbf{\Model regularization:}
    2D example for a 12-parameter fully connected binary network $\sigma( \mathbf{w_2}^\intercal \sigma(\mathbf{w_1}^\intercal \mathbf{x} + \mathbf{b_1}) )$,  where $\sigma(\cdot)$ is a sigmoid nonlinearity. Weights are in $\{ -1, 1 \}$.
    (a) Enumeration of all decision boundaries for 12 binary parameters (4096 = $2^{12}$ combinations).
    (d) Weight combinations and unique solutions when using our \model constraint.
    Using the bi-half works as a regularization, reducing the search-space while retaining the majority of the solutions.
    }
 \label{fig:decision_bound}
\end{figure}

\noindent \textbf{Effect of hyper parameters tuning?} 

\noindent \textbf{Which bit-ratio is preferred?} 
% \subsubsection{\textbf{Exp 2.a:} Which bit-ratio is preferred? }
% - (varying the ppos distribution)
In \fig{bit_epochs}, we evaluate the hyper-parameter $p_{\text{pos}}$ in the Bernoulli prior for Conv2 on Cifar-10 and  Cifar-100.
The x-axis is the probability of the $+1$ connections denoted by $p_{\text{pos}}$ in the Bernoulli prior distribution, while the y-axis denotes the top-1 accuracy values.
% When we fix the pruning ratio, the performance shown by the straight line has a maximum value around the median point where the binary weights over the pruned model are \emph{bi-half} distributed. 
By varying the bit-ratio, the best performance is consistently obtained at the \emph{bi-half} points. 
% The lowest performance appears when $p_{\text{pos}}$ is 0\% or 100\% which means all weights in the subnetwork are set to same value, +1 or -1.  
When there is no other a-priori reason, following the \emph{bi-half} distribution is a good choice. 


% \begin{figure*}[t]
%     \centering
%     \begin{tabular}{c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
%             \includegraphics[width=0.19\textwidth]{fig/exp2/Puttingtogether_3baseline.pdf} & \  
%          \includegraphics[width=0.193\textwidth]{fig/exp2/Varying_bit_rate.pdf} &  \   \  \
%                   \includegraphics[width=0.197\textwidth]{fig/entropy/weight_entropy3baselines.pdf} &   \ 
%                  \includegraphics[width=0.193\textwidth]{fig/entropy/feature_entropy3baselines.pdf}   & \ 
%     % \includegraphics[width=0.194\textwidth]{fig/entropy/feature_entropy3baselines.pdf}

    
%     %  \multicolumn{2}{c}{\ \ \ \ \ \ \ \ \ \  TTQ} \\
%     %  \ \ \ \ \ Conv4 &  \ \ \ \ Conv8  \\
%     \end{tabular}
%     \caption{\small
% %     \textbf{Exp 1 and 2:  Binary 
% % weights distribution for different methods  over the epochs on Cifar-10 using Conv2; Which bit-ratio is preferred?}
% %     On Cifar-10/100 for Conv2 we vary the probabilities of binary values.
%     }
%      \label{fig:TTQ_epochs}
% \end{figure*}



\begin{figure*}[t]
    \centering
    \begin{tabular}{c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
            % \includegraphics[width=0.19\textwidth]{fig/exp2/Puttingtogether_3baseline.pdf} & \  
        %  \includegraphics[width=0.16\textwidth]{fig/exp2/Varying_bit_rate.pdf} &  \   \  \
        %           \includegraphics[width=0.16\textwidth]{fig/entropy/weight_entropy3baselines1.pdf} &   \ 
    \includegraphics[width=0.23\textwidth]{fig/eweight_hitting/Entropy_conv2weightepoch.pdf} & \ \ \                      \includegraphics[width=0.215\textwidth]{fig/entropy/feature_entropy3baselines3.pdf}  & \  \ \ 
    \includegraphics[width=0.19\textwidth]{fig/eweight_hitting/filters_hist_weight.pdf} \ 
    % \includegraphics[width=0.194\textwidth]{fig/entropy/feature_entropy3baselines.pdf}

    
    %  \multicolumn{2}{c}{\ \ \ \ \ \ \ \ \ \  TTQ} \\
    %  \ \ \ \ \ Conv4 &  \ \ \ \ Conv8  \\
    \end{tabular}
    \caption{\small
    Entropy of feature activations before binarization. 
%     \textbf{Exp 1 and 2:  Binary 
% weights distribution for different methods  over the epochs on Cifar-10 using Conv2; Which bit-ratio is preferred?}
%     On Cifar-10/100 for Conv2 we vary the probabilities of binary values.
    }
     \label{fig:bit_epochs}
\end{figure*}



% \begin{figure}[t]
%     \centering
%         \begin{tabular}{ccccc}
%     \includegraphics[width=0.20\textwidth]{fig/exp2/Puttingtogether_3baseline.pdf} &
%         \includegraphics[width=0.205\textwidth]{fig/exp2/Varying_bit_rate.pdf}
%     %  \multicolumn{2}{c}{\ \ \ \ \ \ \ \ \ \  TTQ} \\
%     %  \ \ \ \ \ Conv4 &  \ \ \ \ Conv8  \\
%     \end{tabular}
%     %  \ \   \includegraphics[width=0.492\textwidth]{fig/eweight_hitting/bihalf_sign_flipped_epoch.pdf} \\
%     \caption{\small
%     \textbf{Exp 1 and 2:  Binary 
% weights distribution for different methods  over the epochs on Cifar-10 using Conv2; Which bit-ratio is preferred?}
%     On Cifar-10/100 for Conv2 we vary the probabilities of binary values.
%     % The x-axis shows the prior probability of a positive binary value (\eg +1), which is the hyperparameter $p_{pos}$ of the Bernoulli distribution.
%     % The y-axis denotes the pruning ratio $\rho$.
%     % The color bar indicates the distribution of values for the top-1 accuracy, where dark red is 100\% and dark blue is 0\%.
%     % By varying the probability of pruned weights, the best performance is consistently obtained along the \emph{bi-half} solid line.
%     }
%     \label{fig:app_rescale_prunstratagy}
% \end{figure}

%=========================================================================================
\noindent \textbf{Optimization benefits with bi-half.} 
% \subsubsection{\textbf{Exp 2.b}: \Model optimization benefits.}
The uniform prior over the $-1$ and $+1$ under the Bernoulli distribution regularizes the problem space. This leads to only a subset of possible weight combinations being visited during training.

We illustrate this intuitively on a 2$D$ example for a simple fully-connected neural network with one input layer, one hidden layer, and one output layer in a two-class classification setting.
We consider a 2$D$ binary input vector $\mathbf{x} = [x_1, x_2]^\intercal$, and define the network as: $\sigma( \mathbf{w_2}^\intercal \sigma(\mathbf{w_1}^\intercal \mathbf{x} + \mathbf{b_1}))$, where $\sigma(\cdot)$ is a sigmoid nonlinearity, $\mathbf{w_1}$ is a $[2 \times 3]$ binary weight matrix, $\mathbf{b_1}$ is $[3 \times 1]$ binary bias vector, and $\mathbf{w_2}$ is a $[3 \times 1]$ binary vector.
We group all $12$ parameters as a vector $\mathbf{B}$. 
We enumerate all possible binary weight combinations in $\mathbf{B}$, \ie \ $2^{12}= 4096$, and plot all decision boundaries that separate the input space into two classes as shown in \fig{decision_bound}(a). All possible 4096 binary weights combinations offer only $76$ unique decision boundaries.
In \fig{decision_bound}.(b) the Bernoulli distribution over the weights with equal prior (\model) regularizes the problem space: it reduces the weight combinations to $924$, while retaining $66$ unique solutions.
\todo{Why is it ok to lose some solutions?}




\begin{figure}[t]
\centering
\begin{tabular}{c@{}c@{}c@{}}
    \includegraphics[width=0.23\textwidth]{fig/exp2/Varying_bit_rate.pdf}  & 
    \includegraphics[width=0.24\textwidth]{fig/100time/sorted_index.pdf}   \\ 
    {\small \ \ \  (a) Binary weights entropy} & \
    {\small(b) Varying bit-ratio} \\
    \end{tabular}
    \caption{ \small
    }
 \label{fig:entropybitratio}
\end{figure}




\begin{figure*}[t]
    \centering
    \begin{tabular}{c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
            \includegraphics[width=0.23\textwidth]{fig/100time/Trainingloss.pdf} & \  \ 
         \includegraphics[width=0.23\textwidth]{fig/100time/Trainingacc.pdf} &  \   \  
                  \includegraphics[width=0.23\textwidth]{fig/100time/testloss.pdf} &   \  \
                 \includegraphics[width=0.23\textwidth]{fig/100time/testacc.pdf}   & \  \ 
                                %   \includegraphics[width=0.20\textwidth]{fig/100time/sorted_index.pdf}   & \  \ 
                 
    % \includegraphics[width=0.194\textwidth]{fig/entropy/feature_entropy3baselines.pdf}

    
    %  \multicolumn{2}{c}{\ \ \ \ \ \ \ \ \ \  TTQ} \\
    %  \ \ \ \ \ Conv4 &  \ \ \ \ Conv8  \\
    \end{tabular}
    \caption{\small
%     \textbf{Exp 1 and 2:  Binary 
% weights distribution for different methods  over the epochs on Cifar-10 using Conv2; Which bit-ratio is preferred?}
%     On Cifar-10/100 for Conv2 we vary the probabilities of binary values.
    }
     \label{fig:runing100times}
\end{figure*}



\subsection{
Exp 3: Different architectures on Cifar-100
}
In \fig{}, we study the effectiveness of the proposed methods for different architectures on Cifar-100 dataset. 


\begin{table}[t]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\resizebox{1\linewidth}{!}{
	 \setlength{\tabcolsep}{0.95mm}{
	   	\begin{tabular}{lcccccc}
    	\toprule
		 	    Method 
		 	    % &  \multicolumn{2}{c}{Storage Cost (Mbit)} & & \multicolumn{2}{c}{Accuracy (\%)} \\
			    & Conv2  & Conv4 &  Conv6  & Conv8 \\\midrule		
		        Sign           & 77.86$\pm$ 0.69  & 86.49$\pm$ 0.24 &  88.51$\pm$ 0.35 &  89.17$\pm$0.26  \\
		        IR-Net     & 78.32$\pm$ 0.25  & 87.20$\pm$ 0.26 &  89.61$\pm$ 0.11 &  90.06$\pm$0.06  \\ 		
			    Ours      & 79.25$\pm$ 0.28  & 87.68$\pm$ 0.32 &  89.92$\pm$ 0.19 &  90.40$\pm$0.17  \\	
			 %   MobileNet~\cite{howard2017mobilenets}       & 105.90  & 0.76 &  65.66$\pm$ 0.09 &45.36$\pm$3.24  \\
		  %      ShuffleNet~\cite{zhang2018shufflenet}      & 33.34   & 0.32 &  71.78$\pm$ 0.28  &  60.25$\pm$0.63  \\
	        \bottomrule
		\end{tabular}
	}
	}
% 	\vspace{0.05in}
	\caption{
	\small
% 	\textbf{Exp 2.1: Storage savings for different architectures.}
	 Accuracy comparison over different methods by training the Conv2/4/6/8 networks on Cifar-10.
}
	\label{tab:convnetacc}
	
\end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{fig/exp2/histogram_new.pdf}
    \caption{\small
    \textbf{Exp 3: Different architectures on CIFAR100.}
    % The x-axis shows the prior probability of a positive binary value (\eg +1), which is the hyperparameter $p_{pos}$ of the Bernoulli distribution.
    % The y-axis denotes the pruning ratio $\rho$.
    % The color bar indicates the distribution of values for the top-1 accuracy, where dark red is 100\% and dark blue is 0\%.
    % By varying the probability of pruned weights, the best performance is consistently obtained along the \emph{bi-half} solid line.
    }
    \label{fig:app_rescale_prunstratagy}
\end{figure*}


% \begin{figure*} [t]
%     \centering
%     \begin{tabular}{@{}c@{}c@{}c@{}@{}c@{}c@{}c@{}}
%     \includegraphics[width=0.237\textwidth]{fig/entropy/weight_entropy3baselines.pdf} & \ \
%     \includegraphics[width=0.232\textwidth]{fig/entropy/feature_entropy3baselines.pdf} & \ \
%     \includegraphics[width=0.24\textwidth]{fig/entropy/filters_hist_weight.pdf} & \ \
%     \includegraphics[width=0.245\textwidth]{fig/entropy/filters_hist_weight.pdf} \\
%     \ \ \ \ \ {Conv2} & \ \  \ \ \ \ \ {Conv4} & \ \ \ \ \ \ \ {Conv6}& \ \ \ \ \ \ \ {Conv8}  \\
%     \end{tabular}
%     \caption{\small
%     \textbf{Exp 2.1: Binarization strategies comparison.}
%     Test accuracy of Conv2/4/6/8 on Cifar-10 when varying the \% pruned weights in each layer.
%     Each curve is the average over five trials.
%     There exist subnetworks that consistently outperform the full binary network.
%     The proposed \emph{bi-half} regularization term helps in finding the best solution.
%     As the networks become deeper, the proposed \emph{Bi-half+OurPrune+Rescale} consistently performs better for all pruning ratios.
%     }
%  \label{fig:shallow_va}
% \end{figure*}


% \begin{figure*}[t]
%     \centering
%     \begin{tabular}{c@{}c@{}c@{}c@{}}
%     %   \multicolumn{2}{c}{\includegraphics[width=0.3\textwidth]{fig/ternary/ternary_percentage_lengend_conv2_1.pdf}} \\
%         %   \multicolumn{2}{c}{\ \ \ \ \ \ \ \ \ \  TWN} \\
%         \includegraphics[width=0.245\textwidth]{fig/entropy/filters_hist_weight.pdf} & \ 
%               \includegraphics[width=0.245\textwidth]{fig/entropy/feature_hist.pdf} & \ 
%              \includegraphics[width=0.245\textwidth]{fig/entropy/feature_hist.pdf} & \ 
%  \includegraphics[width=0.245\textwidth]{fig/entropy/feature_hist.pdf} \\
%             \includegraphics[width=0.22\textwidth]{fig/entropy/weight_entropy3baselines.pdf} & \ 
%          \includegraphics[width=0.22\textwidth]{fig/entropy/weight_entropy3baselines.pdf} & \ 
%          \includegraphics[width=0.22\textwidth]{fig/entropy/weight_entropy3baselines.pdf} & \ 
%     \includegraphics[width=0.215\textwidth]{fig/entropy/feature_entropy3baselines.pdf} 
    
%     %  \multicolumn{2}{c}{\ \ \ \ \ \ \ \ \ \  TTQ} \\
%     %  \ \ \ \ \ Conv4 &  \ \ \ \ Conv8  \\
%     \end{tabular}
%     \caption{\small
%     \textbf{Exp 2: Comparison with ternary strategies.}
%     Ternary weights distribution over the epochs on Cifar-10 using Conv4/6/8.
%     For  TWN method,  the distribution of $+1$ and $-1$ is not well balanced. 
%     TTQ induces lower sparsity as the network gets deeper. 
%     We utilize optimal transport to precisely control the weight distribution throughout the whole training process.
%     }
%      \label{fig:TTQ_epochs}
% \end{figure*}




\begin{table}[t]
	\centering
	    \renewcommand{\arraystretch}{1.2}
		\setlength{\tabcolsep}{1mm}{
	    \resizebox{0.95\linewidth}{!}{
		\begin{tabular}[c]{llcccclccccc}
		\toprule			
        \multirow{1}*{Backbone}  &  \multirow{1}*{Method}&    \multirow{1}*{Bit-width} &   Top-1(\%) & {Top-5(\%) } \\
        & &  (W/A) \\\midrule
		\multirow{10}*{ResNet-18}  & FP & 32/32  &  69.3 &  89.2  \\ % \cmidrule(l){2-5}
    	& ABC-Net & 1/1 &   42.7 &  67.6      \\	
		& XNOR & 1/1  &    51.2&  73.2    \\ 	
		& BNN+& 1/1 &  53.0 & 72.6   \\
		& Least-squares  & 1/1 & 58.9 & 81.4 \\
				& XNOR++ & 1/1 &  57.1 & 79.9  &  \\
		& IR-Net & 1/1 &  58.1 & 80.0  \\
		& RBNN  & 1/1 &   59.9 &   {81.9 }  \\	
% 		& Real2Binary & 1/1 &  60.9 & 83.0  \\
& Sign (ours) & 1/1 &  59.98 & 82.47  \\
		& Ours & 1/1 &  \textbf{60.40}  &   \textbf{82.86}           \\	
	    \midrule
		\multirow{6}*{ResNet-34}  & FP & 32/32  &   73.3 & 91.3   \\ %\cmidrule(l){2-5}
	&	ABC-Net & 1/1  & 52.4 & 76.5 \\
& Bi-Real&  1/1 & 62.2 & 83.9 \\
		& IR-Net  & 1/1 &   {62.9} &   {84.1}  \\
	& RBNN  & 1/1 &   63.1 &   {84.4 }  \\	
        & Ours  & 1/1 & \textbf{64.17} &  \textbf{85.36}    \\
        \bottomrule
		\end{tabular}}}
		    	\vspace{0.05in}
	\caption{\small
	\textbf{Exp 3.1: Comparison with binary networks.}
	Top-1 and Top-5 accuracy on ImageNet.
% 	We prune 80\% of the weights per layer and binarize both weights and activations (W/A).
% 	We compare with a set of state-of-the-art methods and the full precision (FP) models.
% 	The bit-width of our method depends on the predefined pruning ratio $\rho \in (0,1)$.
% 	Our method compares favorably to existing work.
    }
\label{tab:imagnet}
\end{table}




\subsection{Comparison with  state-of-the-art}
For ImageNet, we study the performance of our proposed method using a ResNet-18 and ResNet-34 backbone.
\tab{imagnet} shows a number of state-of-the-art quantization methods over ResNet18 and ResNet-34, including:
ABC-Net~\cite{lin2017towards},
% SQ-BWN ~\cite{dong2017learning},
XNOR~\cite{rastegari2016xnor},
BNN+~\cite{darabi2018bnn+},
% HORQ~\cite{li2017performance},
Bi-Real~\cite{liu2018bi},
% BWHN~\cite{hu2018hashing},
%DoReFa-Net~\cite{zhou2016dorefa},
RBNN~\cite{lin2020rotated},
XNOR++~\cite{bulat2019xnornet},
IR-Net~\cite{qin2020forward}, and
Real2binary \cite{martinez2020training}.
We prune $80\%$ of the weights in each layer which prunes $78.3\%$ and $79.1\%$ weights in total for ResNet-18 and ResNet-34, respectively.
We denote the bit-width for our method as $1+\frac{1}{2}\rho$, since $\rho$ weights are pruned and therefore can take 3 symbols during training, and (1-$\rho$) weights are binary.
For a pruning rate of 80\% corresponds to a bit-width of 1.4.
We use the \emph{Bi-half+OurPrune+Rescale} for our approach.
We can observe that for both weight\slash activation (W/A) bit-width settings on ResNet-18, our method outperforms most other methods by a large margin.
Similar improvements can be observed for ResNet-34.
Our found subnetworks reduce the storage cost $4\times$ compared with the full binary network and although they use a slightly larger bit-width, are more competitive than the state-of-the-art binary networks.

==> experiments.tex <==
\section{Experiments}
%--------------------------------------------------------------------------------------
\noindent \textbf{Datasets and implementation details.} \label{ss}
We evaluate on CIFAR-10, CIFAR-100~\cite{krizhevsky2009learning} and ImageNet~\cite{deng2009imagenet}, for 11 network architectures.
Following~\cite{frankle2018lottery,ramanujan2020s} we evaluate 4 shallow CNNs: Conv2, Conv4, Conv6, and Conv8 with 2/4/6/8 convolutional layers.
We train the shallow models on CIFAR-10 for 100 epochs, with weight decay $1e^{-4}$, momentum 0.9, batch size 128, and initial learning rate 0.1 using a cosine learning rate decay~\cite{loshchilov2016sgdr}.
Following~\cite{qin2020forward} we also evaluate their ResNet-20 architecture and settings on CIFAR-10.
On CIFAR-100, we evaluate our method on 5 different models described below.
We train the CIFAR-100 models for 350 epochs using SGD with weight decay $5e^{-4}$, momentum 0.9, batch size 128, and initial learning rate 0.1 divided by 10 at epochs 150, 250 and 320.
For ImageNet we use ResNet-18 and ResNet-34 trained using SGD with momentum $0.9$, weight decay $1e^{-4}$, and batch size 256.
All our models are trained from scratch without any pre-training.
For the shallow networks we apply our method on all layers, while for the rest we follow~\cite{liu2018bi,qin2020forward}, and apply it on all convolutional and fully-connected layers except the first, last and the downsampling layers. We share all code\footnote{Link to our github source code omitted for review}.

%--------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
\subsection{Exp 1: Motivation for our \emph{bi-half}+pruning}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.36\textwidth]{fig/sign_reg_1.pdf}
    \caption{\small
    \textbf{Exp 1: Motivation for our \emph{bi-half}+pruning.}
    On CIFAR-10 for Conv2 we vary the probabilities of binary values and pruned weights.
    The x-axis shows the prior probability of a positive binary value (\eg +1), which is the hyperparameter $p_{pos}$ of the Bernoulli distribution.
    The y-axis denotes the pruning ratio $\rho$.
    The color bar indicates the distribution of values for the top-1 accuracy, where dark red is 100\% and dark blue is 0\%.
    By varying the probability of pruned weights, the best performance is consistently obtained along the \emph{bi-half} solid line.
    }
    \label{fig:app_rescale_prunstratagy}
\end{figure}
In \fig{app_rescale_prunstratagy}, we evaluate the hyper-parameter $p_{\text{pos}}$ in the Bernoulli prior for Conv2 on CIFAR-10.
The x-axis is the probability of the $+1$ connections denoted by $p_{\text{pos}}$ in the Bernoulli prior distribution, while the y-axis denotes the probability of pruned connections or the pruning ratio $\rho$.
The color bar denotes the distribution of the top-1 accuracy values with dark red being 100\% and dark blue 0\%.
When we fix the pruning ratio, the performance shown by the straight line has a maximum value around the median point where the binary weights over the pruned model are \emph{bi-half} distributed.
By varying the pruning ratio, the best performance is consistently obtained along the \emph{bi-half} solid line. The lowest performance appears when $p_{\text{pos}}$ is 0\% or 100\% which means all weights in the subnetwork are set to same value, +1 or -1.
When there is no other a-priori reason, following the \emph{bi-half} distribution is a good choice.

%--------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
\subsection{Exp 2: Model ablations}
We run ablation studies on the shallow networks (Conv2/4/6/8) on CIFAR-10.
We consider the following approaches:
(i) \emph{Sign}: binary network baseline~\cite{rastegari2016xnor} with weights learned using the $sign$ function without pruning;
(ii) \emph{Bi-half}: using only our \emph{bi-half} prior over the binary weights without pruning;
(iii) \emph{InitPrune}: \emph{sign} baseline without learning weights, with a learnable mask baseline on the initialized values, as developed for non-binary network pruning in~\cite{ramanujan2020s};
(iv) \emph{Sign+OurPrune}: \emph{sign} with our pruning, optimized separately;
(v) \emph{Bi-half+OurPrune}: our full model jointly optimizing pruning and the \emph{bi-half} binary distribution;
(vi) \emph{Bi-half+OurPrune+Rescale}: using the $\alpha$ rescaling as explained in the method;
(vii) \emph{Sign$\rightarrow$Prune$\rightarrow$Sign} uses a typical pruning algorithm as in ~\cite{han2016deep} where we train a model, prune it and fine-tune it or use rewinding;
(viii) \emph{Sign$\rightarrow$InitPrune}i: separately optimizes the binary connections and the pruning mask;
(ix) \emph{InitPrune$\rightarrow$Sign}: first finds a subnetwork by \emph{InitPrune} and then trains the binary connections of the subnetwork with \emph{sign} quantization.

%--------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
\subsection{Exp 2.1: Ablation of model modules}
\begin{figure*} [t]
    \centering
    \begin{tabular}{@{}c@{}c@{}c@{}@{}c@{}c@{}c@{}}
    \multicolumn{4}{c}{
    \includegraphics[width=0.88\textwidth]{fig/shallow/lengend_prune1.pdf}}\\
    \includegraphics[width=0.24\textwidth]{fig/shallow/acc_pruneweight_conv2.pdf} & \ \
    \includegraphics[width=0.24\textwidth]{fig/shallow/acc_pruneweight_conv4.pdf} & \ \
    \includegraphics[width=0.24\textwidth]{fig/shallow/acc_pruneweight_conv6.pdf} & \ \
    \includegraphics[width=0.24\textwidth]{fig/shallow/acc_pruneweight_conv8.pdf} \\
    \ \ \ \ \ {Conv2} & \ \  \ \ \ \ \ {Conv4} & \ \ \ \ \ \ \ {Conv6}& \ \ \ \ \ \ \ {Conv8}  \\
    \end{tabular}
    \caption{\small
    \textbf{Exp 2.1: Binarization strategies comparison.}
    Test accuracy of Conv2/4/6/8 on CIFAR-10 when varying the \% pruned weights in each layer.
    Each curve is the average over five trials.
    There exist subnetworks that consistently outperform the full binary network.
    The proposed \emph{bi-half} regularization term helps in finding the best solution.
    As the networks become deeper, the proposed \emph{Bi-half+OurPrune+Rescale} consistently performs better for all pruning ratios.
    }
 \label{fig:shallow_va}
\end{figure*}
%---------------------------------------------------------------------
\noindent\textbf{Binarization strategies comparison.}
Here, we consider different binarization strategies on CIFAR-10 using Conv2/4/6/8.
Results in \fig{shallow_va} show that all 4 CNNs behave similarly, yet accuracy increases as the network becomes deeper.
The proposed \emph{bi-half} regularization term helps in finding the best solution, and consistently outperforms using the \emph{sign}.
The pruned variants do better, both when quantizing using \emph{sign} and \emph{bi-half}.
Too aggressive pruning reduces performance due to exploding gradients~\cite{glorot2010understanding, he2015delving}.
With the \emph{bi-half} regularization, the \emph{Bi-half+OurPrune} outperforms \emph{Sign+OurPrune} for all shallow networks, except for large pruning ratios on the Conv2 and Conv4 networks.
Pruning reduces the search space considerably on the very shallow networks,
therefore the additional \emph{bi-half} regularization does not aid the optimization further.
\fig{shallow_va} shows that rescaling helps against exploding gradients, and therefore our \emph{Bi-half+OurPrune+Rescale} performs the best across all pruning ratio.
To fairly evaluate the performance of the proposed rescaling factor, we evaluated this rescaling for both methods: \emph{Sign+OurPrune} and \emph{Sign+OurPrune}.

%---------------------------------------------------------------------
\smallskip\noindent\textbf{Pruning strategies comparison.}
We consider multiple pruning strategies.
All pruning strategies rewind the learning rate schedule to retrain the pruned subnetwork as in~\cite{renda2020comparing}.
In \fig{prunstratagy}, we see that the \emph{Sign$\rightarrow$Prune$\rightarrow$Sign} under-performs due to the distribution of the binary connections $+1$\slash $-1$ being unbalanced by the pruning.
The \emph{Sign$\rightarrow$InitPrune} is consistently better than \emph{InitPrune}: a good initialization achieved by the \emph{sign} quantization helps in finding accurate subnetwork.
\emph{InitPrune$\rightarrow$Sign} performs worse than \emph{Sign$\rightarrow$Prune$\rightarrow$Sign} because applying the $sign$ followed by pruning can capture some information about the real-valued weights which is helpful for pruning.
In contrast, \emph{InitPrune} searches for subnetworks without learning the real-valued weights, yet applying $sign$ after pruning is equivalent to training a small network from scratch.
Our proposed method \emph{Bi-half+OurPrune+Rescale} consistently outperforms other pruning strategies.
\begin{figure}[t]
\centering
    \begin{tabular}{c@{}c}
    \multicolumn{2}{c}{\includegraphics[width=0.45\textwidth]{fig/shallow/rewind_lengend1.pdf}} \\
    \includegraphics[width=0.22\textwidth]{fig/shallow/Rewind_accvsepoch_prune05.pdf} &
    \includegraphics[width=0.22\textwidth]{fig/shallow/Rewind_acc_pruneweight.pdf}
    \\
    \end{tabular}
    \caption{\small
    \textbf{Exp 2.1: Pruning strategies comparison.}
    Comparison on CIFAR-10 of different pruning strategies using learning rate rewinding~\cite{renda2020comparing} using Conv6:
    Our proposed \emph{Bi-half+OurPrune} method performs the best.
    }
     \label{fig:prunstratagy}
\end{figure}

%--------------------------------------------------------------------------------------
\begin{comment}
% This experiments does not add much info.
\smallskip\noindent \textbf{Memory savings for different strategies.}
As demonstrated in \cite{rastegari2016xnor}, when binarizing both weights and activations a 58$\times$ speedup on CPUs is achieved.
Here we evaluate our method with binarized activations.
Following \cite{courbariaux2016binarized, rastegari2016xnor}, we use the $sign$ function as the activation function in the forward pass, and in backward pass we use gradient clipping -- the gradient is passed through a hard $tanh$.
In \tab{three_nets} we use three different architectures: ResNet-20, ResNet-18 and ResNet-34.
The $1/32$ and $1/1$ indicate the bit-width for weights and for activations.
$1/1$ means that we quantize both the weights and the activations to 1-bit.
We conclude that our methods can find a subnetwork that outperforms the full binary network.
\begin{table*}[!t]
	\centering
	    \renewcommand{\arraystretch}{1.0}
	    \setlength{\tabcolsep}{3mm}{
 	    \resizebox{1\linewidth}{!}{
		\begin{tabular}[c]{lcccccccccccc}
			\toprule
		 	  \multirow{2}*{Method}&    \multirow{2}*{Memory saving} &  & \multicolumn{2}{c}{ ResNet-20 (CIFAR-10)}  & & \multicolumn{2}{c}{ ResNet-18 (CIFAR-100)}  & & \multicolumn{2}{c}{ ResNet-34 (CIFAR-100)}\\ \cline{4-5} \cline{7-8} \cline{10-11} \\
		 	    FP  & 1 $\times$ & &  \multicolumn{2}{c}{ 92.21$\pm$ 0.18 } & &  \multicolumn{2}{c}{ 78.59$\pm$ 0.44 }   & &  \multicolumn{2}{c}{ 79.37$\pm$ 0.02 }  \\
                \midrule
                & & &  1/32  & 1/1 & &  1/32  & 1/1 & &   1/32  & 1/1  \\ \cline{4-11}	 	
		        Sign & $\sim$ 32$\times$  &  & 90.29$\pm$ 0.18 &  85.61$\pm$ 0.34 &  &  75.56$\pm$0.09 &  71.28$\pm$0.11 && 76.99 $\pm$ 0.03  & 72.48 $\pm$ 0.01\\
			    Bi-half  & $\sim$ 32$\times$ &  & 90.51$\pm$ 0.15 &  85.89$\pm$ 0.16  &  &  76.29$\pm$ 0.14 &  71.60$\pm$0.04  && 77.21$\pm$0.16 & 72.82 $\pm$ 0.05\\	
		        Sign+OurPrune  & $\sim$ 160$\times$ & &   90.92$\pm$ 0.19&  86.12$\pm$ 0.24 & &    76.78$\pm$ 0.08 & 71.95$\pm$0.19 && \textbf{78.215$\pm$0.03} & 73.09 $\pm$ 0.25 \\ 	
		 	    Bi-half+OurPrune &  $\sim$ 160$\times$ &  & 90.81$\pm$ 0.21 &86.49 $\pm$ 0.29 &  & 76.43$\pm$ 0.12 &\textbf{72.63$\pm$0.10}  && 77.97$\pm$0.08 & 73.71 $\pm$ 0.01  \\
			    {Bi-half+OurPrune} & \multirow{2}{*}{$\sim$ 160$\times$} & \multirow{2}{*}{} & \multirow{2}{*}{\textbf{91.03$\pm$ 0.17}} &\multirow{2}{*}{\textbf{ 86.80$\pm$ 0.13}} & & \multirow{2}{*}{76.57$\pm$ 0.31} & \multirow{2}{*}{72.56$\pm$0.11 } & &
			    \multirow{2}{*}{77.82$\pm$0.19} & \multirow{2}{*}{\textbf{73.83 $\pm$ 0.05}}\\
			   + Rescale & & & & & & & & & \\
            \bottomrule
		\end{tabular}}}
	\caption{\small
	    \textbf{Exp 2.1: Memory savings for different strategies.}
	    Top-1 accuracy on CIFAR-10 and CIFAR-100: Results averaged over 3 runs.
	    We prune $80\%$ of weights per layer in this setting.
	    We show different pruning and quantization approaches compared to the full-precision (FP) baseline.
	    Our method is successful at fining an accurate and small subnetwork.
	    }
	\label{tab:three_nets}
	\vspace{-0.1in}
\end{table*}
\end{comment}

%------------------------------------------------------------------------------------

%------------------------------------------------------------------------------------
\smallskip\noindent \textbf{Comparison with ternary strategies.}
\tab{TTQ_TWN} compares our \emph{bi-half} + pruning method with different ternary strategies on Conv2/4/6/8.
TWN~\cite{li2016ternary} uses two symmetric thresholds, and a scaling factor to quantize the full precision weights into ternary weights.
TTQ~\cite{zhu2017trained} introduces two trainable full-precision scaling coefficients to adjust the ternary assignment.
When compared to our method, both TWN and TTQ induce a lower sparsity level while obtaining similar accuracy.
\fig{TTQ_epochs} shows the distribution of $-1$, $0$ and $+1$ on CIFAR-10 for TWN~\cite{li2016ternary}, TTQ~\cite{zhu2017trained} and our method.
In the case of TWN, the network sparsity increases during the training and it converges to $\sim$60\% zeros, $\sim$15\% positive values and $\sim$25\% negative values.
The unbalanced ternary distribution leads the performance degradation as shown in \fig{app_rescale_prunstratagy}.
% TWN assumes the  continuous-valued weights obey uniform or normal distribution. As training the  continuous-valued weights change   computing the thresholds. when the normalization layers are absent.  The unbalanced distribution over positive and negative values will Since the shallow networks do not use normalization layers, we
% The interesting result is that the
TTQ relies on trainable scaling coefficients to balance the distribution of $-1$ and $+1$, and it converges to $\sim$20\% zeros, and an equal percentage of positive and negative values: $\sim$40\%.
We rely on optimal transport to precisely control the weight distribution, which remains fixed throughout training.   More experiments are given in supplementary material.
\begin{table}
	\centering
	\renewcommand{\arraystretch}{1.1}
	\resizebox{1\linewidth}{!}{
	 \setlength{\tabcolsep}{1.0mm}{
	   	\begin{tabular}{lccccccccc}
    	\toprule
		 	    Backbones   &  \multicolumn{2}{c}{TWN~\cite{li2016ternary}} & & \multicolumn{2}{c}{TTQ~\cite{zhu2017trained} }& & \multicolumn{2}{c}{Ours}  \\
			    & Acc.  & Sparsity  & &  Acc. & Sparsity & &  Acc. & Sparsity  \\\midrule		
		        Conv2          & 72.39  & 0.59  && 79.45 & 0.22 &&  79.76 & 0.80 \\
		        Conv4    & 79.92  & 0.49 && 87.78 & 0.24 && 88.64 & 0.80 \\ 		
			    Conv6       & 80.63 & 0.51  && 89.23 &  0.25 && 90.73 & 0.80  \\	
			    Conv8       & 81.42 & 0.55 && 90.06 & 0.13 && 91.236 & 0.80  \\
	        \bottomrule
		\end{tabular}
	}
	}
	\vspace{0.05in}
	\caption{\small
	\textbf{Exp 2.1: Comparison with ternary strategies.}
    Accuracy when compared with different ternary networks of Conv2/4/6/8 on Cifar-10.
    Both TWN and TTQ induce lower sparsity.
    Our method can achieve better performance with higher sparsity.
    (We use the code released by the authors.)
    }
	\label{tab:TTQ_TWN}
\end{table}
\begin{figure}[t]
    \centering
    \begin{tabular}{c@{}c@{}c@{}}
       \multicolumn{3}{c}{\includegraphics[width=0.3\textwidth]{fig/ternary/ternary_percentage_lengend_conv2_1.pdf}} \\
    \includegraphics[width=0.172\textwidth]{fig/ternary/TWNpercentage_allepoch_conv2.pdf} &
    \includegraphics[width=0.146\textwidth]{fig/ternary/ternary_percentage_allepoch_conv2_1.pdf} &
    \includegraphics[width=0.146\textwidth]{fig/ternary/ternary_percentage_ours_conv2_1.pdf} \\
     \ \ \ \ \ TWN &  \ \ \ \ {TTQ} & \ \ \ \ Ours  \\
    \end{tabular}
    \caption{\small
    \textbf{Exp 2.1: Comparison with ternary strategies.}
    Ternary weights distribution over the epochs on CIFAR-10 using Conv2.
    For TWN we observe that as training proceeds, the sparsity gets higher $\sim$60\%, and the positive and negative percentages reduce to $\sim$15\% and $\sim$25\%; where the distribution of $+1$ and $-1$ is not well balanced.
    TTQ introduces trainable scaling coefficients to help balancing the distribution of $-1$ and $+1$, and it achieves a $\sim$20\% sparsity, and $\sim$40\% of positives and negatives.
    We utilize optimal transport to precisely control the weight distribution throughout the whole training process.
    }
     \label{fig:TTQ_epochs}
\end{figure}


%--------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
\subsection{Exp 2.2: Ablation of hyperparameters}
\noindent\textbf{Effect of rescaling in initialization.}
In \fig{rescale} we show results for Conv4/8 (Additional rescaling experiments for Conv2/6 are in the Appendix).
Adding the rescaling factor does not improve the accuracy on the \emph{InitPrune} and \emph{Sign+OurPrune} methods, since the scaling cannot guarantee the activation variance in the forward pass to be close to 1.
Rescaling benefits our method the most.
\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \multicolumn{2}{c}{\includegraphics[width=0.45\textwidth]{fig/shallow/RescaleLengend1.pdf}} \\
    \includegraphics[width=0.22\textwidth]{fig/shallow/Scalemethodacc_pruneweight_conv4.pdf} &
    \includegraphics[width=0.21\textwidth]{fig/shallow/Scalemethodacc_pruneweight_conv8.pdf} \\
    \end{tabular}
    \caption{\small
    \textbf{Exp 2.2: Effect of rescaling in initialization.}
    On CIFAR-10 using Conv4/8:
    The rescaled methods are shown with solid lines, and non-rescaled methods are shown with dashed lines. Rescaling benefits our method the most.
    }
     \label{fig:rescale}
\end{figure}

%--------------------------------------------------------------------------------------

\smallskip\noindent \textbf{Effect of pruning ratio.}
In \fig{pruning} we test the effect of pruning rations on different architectures.
We consider 5 different architectures: VGG16~\cite{simonyan2014very},  ResNet34~\cite{he2016deep}, InceptionV3~\cite{szegedy2016rethinking}, ShuffleNet~\cite{zhang2018shufflenet} and MobileNet~\cite{howard2017mobilenets}, on CIFAR-100.
We increase the pruning rate from $0\%$ all the way up to $96\%$ for Resnet-18 and Resnet-34 on CIFAR-100, when quantizing both weights and activations.
Interestingly, for Resnet-34, pruning $96\%$ gives a similar performance to the full binary network.
The right side of \fig{pruning} shows the accuracy for different percentages of pruned weights.
The  VGG16,  ResNet34 and InceptionV3 have many redundant parameters, thus our method with a pruning ratio of 80\% over each layer outperforms the full binary networks.
It is difficult to quantize the lightweight models, ShuffleNet and MobileNet, as their capacity is already limited.

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=0.215\textwidth]{fig/resnet18/1w_1a_prunemore_resnet18_cifa100_1.pdf}   &
    \includegraphics[width=0.215\textwidth]{fig/resnet18/Diff_netmore_resnet18_cifa100_1.pdf}  \\
    \end{tabular}
    \caption{\small
    \textbf{Exp 2.2: Effect of pruning ratio.}
    $Left$: Pruning rates on CIFAR-100 varying from $0\%$ to $96\%$.
    For Resnet-34, we can prune $96\%$ of the weights without accuracy loss.
    $Right$: Accuracy on CIFAR-100 for our method using VGG16, ResNet34, InceptionV3, ShuffleNet and MobileNet.
    The larger models benefit more from our joint pruning and \emph{bi-half} regularization.
    }
     \label{fig:pruning}
\end{figure}

%-------------------------------------------------------------------------------------------
\smallskip\noindent \textbf{Storage savings for different architectures.}
We evaluate our method on CIFAR-100 over 5 different architectures: VGG16~\cite{simonyan2014very},  ResNet34~\cite{he2016deep}, InceptionV3~\cite{szegedy2016rethinking}, ShuffleNet~\cite{zhang2018shufflenet} and MobileNet~\cite{howard2017mobilenets}, where the last two models are lightweight networks.
In \tab{storage} we compute the memory usage for the 5 backbone architectures.
The memory usage is calculated as a summation of 32 bits for the real-valued parameters, and 1 bit for binary parameters.
Our method can compress the models up to $150\times$.
We can compress InceptionV3 from $714.18$ Mbit to $4.65$ Mbit without performance decrease, but rather a performance increases from $79.70\%$ to $80.34\%$.
This indicates that instead of designing a lightweight model, it is more effective to search for an optimal subnetwork within a larger model.
\begin{table}
	\centering
	\renewcommand{\arraystretch}{1.1}
	\resizebox{1\linewidth}{!}{
	 \setlength{\tabcolsep}{0.9mm}{
	   	\begin{tabular}{lcccccc}
    	\toprule
		 	    Backbones   &  \multicolumn{2}{c}{Storage Cost (Mbit)} & & \multicolumn{2}{c}{Accuracy (\%)} \\
			    & Original  & Ours & & Original  & Ours \\\midrule		
		        VGG16~\cite{simonyan2014very}           & 1088.09 & 7.14  && 73.88$\pm$0.50 & 71.33$\pm$0.08  \\
		        InceptionV3~\cite{szegedy2016rethinking}     & 714.18  & 4.65 && 79.70$\pm$ 0.06 & 80.34$\pm$0.06 \\ 		
			    ResNet34~\cite{he2016deep}        & 682.51  & 4.46 &&  79.37$\pm$ 0.02 &  77.89$\pm$0.19  \\	
			    MobileNet~\cite{howard2017mobilenets}       & 105.90  & 0.76 &&  65.66$\pm$ 0.09 &45.36$\pm$3.24  \\
		        ShuffleNet~\cite{zhang2018shufflenet}      & 33.34   & 0.32 & & 71.78$\pm$ 0.28  &  60.25$\pm$0.63  \\
	        \bottomrule
		\end{tabular}
	}
	}
	\vspace{0.05in}
	\caption{\small
	\textbf{Exp 2.2: Storage savings for different architectures.}
	Comparison of storage cost of different backbone architectures on CIFAR-100.
    We prune 80\% of weights.
	We can substantially reduce the memory costs (up to $150\times$ for InceptionV3) and still outperform the original model. }
	\label{tab:storage}
	
\end{table}

%-------------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
\section{Exp 3: Comparison with state-of-the art}
\begin{table*}
	\centering
	    \renewcommand{\arraystretch}{1.05}
		\setlength{\tabcolsep}{3.5mm}{
	    \resizebox{0.99\linewidth}{!}{
		\begin{tabular}[c]{llcccclccccc}
		\toprule			
        \multirow{1}*{Backbone}  &  \multirow{1}*{Method}&    \multirow{1}*{Bit-width} &   Top-1(\%) & {Top-5(\%) } &  & \multirow{1}*{Method}&    \multirow{1}*{Bit-width} &   Top-1(\%) & {Top-5(\%) } \\
        & &  (W/A) & & & & &  (W/A) & & \\\midrule
		\multirow{9}*{ResNet-18}  & FP & 32/32  &  69.3 &  89.2  & & FP & 32/32  &  69.3 &  89.2 \\ \cmidrule(l){2-10}
    	& ABC-Net~\cite{lin2017towards} & 1/1 &   42.7 &  67.6   & & SQ-BWN~\cite{dong2017learning}  & 1/32 &  58.4 &  81.6    \\	
		& XNOR~\cite{rastegari2016xnor} & 1/1  &    51.2&  73.2  & & BWN~\cite{rastegari2016xnor}   &  1/32  &    60.8&  83.0  \\ 	
		& BNN+~\cite{darabi2018bnn+}& 1/1 &  53.0 & 72.6    & & HORQ~\cite{li2017performance}   &  1/32  &    61.3&  83.2  \\
		& Bi-Real~\cite{liu2018bi} & 1/1 &  56.4 & 79.5  & & BWHN~\cite{hu2018hashing}   &  1/32 &   64.3&  85.9\\	
		& Least-squares \cite{pouransari2020least} & 1/1 & 58.9 & 81.4 & &
		Least-squares \cite{pouransari2020least} & 1/32 & 66.1 & 86.5 \\
		& IR-Net~\cite{qin2020forward} & 1/1 &  58.1 & 80.0  & &
		IR-Net~\cite{qin2020forward}   &  1/32 &    66.5&  86.8 \\
		& XNOR++~\cite{bulat2019xnornet} & 1/1 &  57.1 & 79.9  &  \\
		& Real2Binary~\cite{martinez2020training} & 1/1 &  60.9 & 83.0  & \\
		& Ours & $1+\frac{1}{2}\rho$/$1$ &  \textbf{61.7}  &   \textbf{84.1}         & & Ours   &  $1+\frac{1}{2}\rho$/32  &  \textbf{67.0} &  \textbf{87.6}   \\	
	    \midrule
		\multirow{3}*{ResNet-34}  & FP & 32/32  &   73.3 & 91.3  & & FP & 32/32  &   73.3 & 91.3 \\ \cmidrule(l){2-10}
		& IR-Net~\cite{qin2020forward}  & 1/1 &   {62.9} &   {84.1} & & IR-Net~\cite{qin2020forward} & 1/32 &  \textbf{70.4} &  89.5 \\
        & Ours  & $1+\frac{1}{2}\rho$/$1$ & \textbf{65.2} &  \textbf{86.4}  & & Ours  & $1+\frac{1}{2}\rho$/32 &  {70.0} &  \textbf{89.7}   \\
        \bottomrule
		\end{tabular}}}
		    	\vspace{0.05in}
	\caption{\small
	\textbf{Exp 3.1: Comparison with binary networks.}
	Top-1 and Top-5 accuracy on ImageNet.
	We prune 80\% of the weights per layer and binarize both weights and activations (W/A).
	We compare with a set of state-of-the-art methods and the full precision (FP) models.
	The bit-width of our method depends on the predefined pruning ratio $\rho \in (0,1)$.
	Our method compares favorably to existing work.
    }
\label{tab:imagnet}
\end{table*}

%-------------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
\subsection{Exp 3.1: Comparison with binary networks}
For ImageNet, we study the performance of our proposed method using a ResNet-18 and ResNet-34 backbone.
\tab{imagnet} shows a number of state-of-the-art quantization methods over ResNet18 and ResNet-34, including:
ABC-Net~\cite{lin2017towards},
SQ-BWN ~\cite{dong2017learning},
XNOR, and BWN~\cite{rastegari2016xnor},
BNN+~\cite{darabi2018bnn+},
HORQ~\cite{li2017performance},
Bi-Real~\cite{liu2018bi},
BWHN~\cite{hu2018hashing},
%DoReFa-Net~\cite{zhou2016dorefa},
XNOR++~\cite{bulat2019xnornet},
IR-Net~\cite{qin2020forward}, and
Real2binary \cite{martinez2020training}.
We prune $80\%$ of the weights in each layer which prunes $78.3\%$ and $79.1\%$ weights in total for ResNet-18 and ResNet-34, respectively.
We denote the bit-width for our method as $1+\frac{1}{2}\rho$, since $\rho$ weights are pruned and therefore can take 3 symbols during training, and (1-$\rho$) weights are binary.
For a pruning rate of 80\% corresponds to a bit-width of 1.4.
We use the \emph{Bi-half+OurPrune+Rescale} for our approach.
We can observe that for both weight\slash activation (W/A) bit-width settings on ResNet-18, our method outperforms most other methods by a large margin.
Similar improvements can be observed for ResNet-34.
Our found subnetworks reduce the storage cost $4\times$ compared with the full binary network and although they use a slightly larger bit-width, are more competitive than the state-of-the-art binary networks.

%-----------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------
\subsection{Exp 3.2: Comparison with ternary and 2-bit networks}
\tab{ternary} shows state-of-the-art ternary and 2-bit quantization methods over ResNet18 and ResNet-34, including:
DoReFa~\cite{zhou2016dorefa},
TWN~\cite{li2016ternary},
SQ-TWN~\cite{dong2017learning},
SOWQT~\cite{he2019simultaneously},
HWGQ~\cite{cai2017deep},
Least-squares \cite{pouransari2020least} and
LQ~\cite{zhang2018lq}.
Given that $\rho$ weights during training can take 3 symbols and $1-\rho$ weights are consistently binary, for our method we define the bit-width by $1{+}\frac{1}{2}\rho$, where $\rho$ is the pruning ratio which we set to 80\% and corresponds to a bit-width of 1.4. This is slightly lower then ternary and 2-bit networks.
For the ResNet-18 when quantizing only the weights, our method outperforms existing ternary networks. When quantizing both weights and activations our results are on part with state-of-the-art ternary and 2-bit networks.

\begin{table}
	\centering
	    \renewcommand{\arraystretch}{1.05}
		%\setlength{\tabcolsep}{3.5mm}
		{
	    \resizebox{0.99\linewidth}{!}{
		\begin{tabular}[c]{llcccc}
		\toprule			
        \multirow{1}*{Backbone}  &  \multirow{1}*{Method}&    \multirow{1}*{Bit-width} &   Top-1(\%) & {Top-5(\%) }  \\
        & &  (W/A) & &  \\\midrule
		\multirow{4}*{ResNet-18}  & FP & 32/32  &  69.3 &  89.2   \\ \cmidrule(l){2-5}
	    & SOWQT~\cite{he2019simultaneously} & T/32 &  66.0 & 86.7 \\
	    & TWN~\cite{li2016ternary} &  T/32  &   60.1 &  82.9\\
	    & SQ-TWN~\cite{dong2017learning} &  T/32  &   63.8 &  85.7\\
	    & Ours  & T/32 & \textbf{67.0} &  \textbf{87.6}  \\
	   \cmidrule(l){2-5}
	   	& DoReFa~\cite{zhou2016dorefa} &  2/2    & 62.6 & {84.4}  \\
	   	& HWGQ~\cite{cai2017deep} & 1/2 & 59.6 & 82.2 \\
		& LQ~\cite{zhang2018lq} & 1/2 & 62.6 & 84.3 \\
		& Least-squares~\cite{pouransari2020least} & 1/T &  62.0 & 83.6\\
		& Ours & $1+\frac{1}{2}\rho$/$1$ & {61.7}  &  {84.1} \\		
        \midrule
		\multirow{1}*{ResNet-34}  & FP & 32/32  &   73.3 & 91.3 \\ \cmidrule(l){2-5}
		% & Ours  & 1/1 & \textbf{65.21} &  \textbf{86.43} \\ \cmidrule(l){2-5}
		& SOWQT~\cite{he2019simultaneously} & T/32 &  70.8 & 89.9 \\
		& Ours  & $1+\frac{1}{2}\rho$/32 &  {70.0} &  {89.7} \\
        \bottomrule
		\end{tabular}}}
		\vspace{0.05in}
	\caption{\small
	\textbf{Exp 3.2: Comparison with ternary and 2-bit networks.}
	Top-1 and Top-5 accuracy on ImageNet. We denote ternary bit-width with a ``T".
	The bit-width of our method depends on the  pruning ratio $\rho \in (0,1)$.
	We outperform existing ternary methods when quantizing only the wights, and are on par with existing 2-bit and ternary work when quantizing both weights and activations.
    }
\label{tab:ternary}
\end{table}

%-------------------------------------------------------------------------------------------


==> method.tex <==
\section{Masked {bi-half} binary weights}
\label{approach}

\begin{figure*}[t]
\centering
\begin{tabular}{cc}
    {(a) Full binary network} &
    {(b) Pruned subnetwork} &
    {(c) \emph{Bi-half} subnetwork} \\
    \includegraphics[width=0.25\textwidth]{fig/toy/Onecolor_prune0.pdf} &
    \includegraphics[width=0.25\textwidth]{fig/toy/Onecolor_prune1_nohalf.pdf} &
    \includegraphics[width=0.25\textwidth]{fig/toy/blackcolor_figure_half_half.pdf} \\
    \scriptsize{Weight combinations: 512.} &
    \scriptsize{Weight combinations: 2304.} &
    \scriptsize{Weight combinations: 630.}  \\
    \scriptsize{Unique solutions: 30.} &
    \scriptsize{Unique solutions: 109.} &
    \scriptsize{Unique solutions: 98.}  \\[3px]
    {(d) \Model with no pruning} &
    {(e) Ternary space} &
    {(f) Solution space } \\
    \includegraphics[width=0.25\textwidth]{fig/toy/Onecolor_prune0.pdf} &
    \includegraphics[width=0.25\textwidth]{fig/toy/ternary_figure_half_half.pdf} &
    \includegraphics[width=0.25\textwidth]{fig/toy/log_solution_unique} \\
    \scriptsize{Weight combinations: 252.} &
    \scriptsize{Weight combinations: 19683.} &
    \scriptsize{Unique/possible solutions}\\
    \scriptsize{Unique solutions: 30.} &
    \scriptsize{Unique solutions: 431.} &
    \scriptsize{vs pruned weights.} \\
\end{tabular}
    \caption{ \small
2D example for a 9-parameter fully connected binary network $\sigma( \mathbf{w}^\intercal \tanh(\mathbf{W}^\intercal \mathbf{x} + \mathbf{b}) + c)$,  where $\sigma$ is a sigmoid nonlinearity. Weights are in $\{ -1, 1 \}$ or $0$ when pruned.
    (a) Enumeration of all decision boundaries for 9 binary parameters (512 = $2^9$ combinations).
    (b) The same network for all possibilities of having 1 out of the 9 weights pruned ($2304 = 9*2^8$ combinations).
    (c) Having 1 out of the 9 weights pruned  and constraining the binary weights to the \emph{bi-half} distribution, \ie: the 9 weights sum to $0$, ($630 =9*C_8^4$ combinations, where $C$ is the combination notation). The black lines are the only 11 decision boundaries lost due to the \emph{bi-half} prior.
    (d) Weight combinations and unique solutions when using the \emph{bi-half} regularization without pruning.
    (e) The solutions space and weight combinations when considering 3 symbols: $3^9$.
    %(f) The \emph{bi-half} regularization applied over ternary solution space.
    (f) Number of possible solutions and number of unique solutions vs the number of pruned weights.
    Comparing (a) and (b) illustrates that pruning increases the representational power of the network.
    (c) and (d) show that the half-half binary weight distribution (\emph{bi-half}) strongly constrains the search space without greatly affecting the representational power as measured by the number of unique solutions.
   % \slp{Bi-half over ternary does not say anything to me? I wont refer to it in the text because it does not say anything.}    
   }
 \label{fig:decision_bound}
\end{figure*}


%--------------------------------------------------------------------------
\noindent \textbf{Illustrative 2D example.} To help our explanation, we show a 2$D$ example for a simple fully-connected neural network with one input layer, one hidden layer, and one output layer in a two-class classification setting.
We consider a 2$D$ binary input vector $\mathbf{x} = [x_1, x_2]^\intercal$,
a $2 \times 2$ binary weight matrix $\mathbf{W}$, and a 2$D$ binary bias vector $\mathbf{b}$ as the hidden layer, followed by a $\tanh$ nonlinear activation, and an output layer composed of a $2 \times 1$ binary weight and a binary bias $c$.
Thus, the output of the network is $\sigma( \mathbf{w}^\intercal \tanh(\mathbf{W}^\intercal \mathbf{x} + \mathbf{b}) + c)$,  where $\sigma$ is a sigmoid nonlinearity.
We group all $9$ parameters as a vector $\mathbf{B}$. We enumerate all possible binary weight combinations in $\mathbf{B}$, \ie \ $2^9 = 512$, and plot all decision boundaries that separate the input space into two classes as shown in \fig{decision_bound}(a). All possible 512 binary weights combinations offer only $30$ unique decision boundaries.

%--------------------------------------------------------------------------
%--------------------------------------------------------------------------
%--------------------------------------------------------------------------
\subsection{Pruning binary weights increases search space}
In our 2$D$ example, if we \emph{randomly} select 1 out of 9 weights of $\mathbf{B}$ and prune it, we have $9$ possible sub-networks with $9*2^8 = 2,304$  binary weight combinations.
All $109$ unique decision boundaries are shown in \fig{decision_bound}(b). Comparing the full binary network in \fig{decision_bound}(a) with its pruned variant in \fig{decision_bound}(b) illustrates that pruning a single binary weight increases the number of unique decision boundaries and thus increases the solution space.

Pruning increases the search space dramatically for certain pruning ratios $\rho$.
Given $n$ binary connections in $\mathbf{B}$, when pruning weights by a ratio $\rho$ we have $C^{n\rho}_n * 2^{n(1-\rho)}$ different network parameterizations, where $C^\cdot_\cdot$ is the combination notation, and the maximum is achieved when $\rho = 1/3$.
In \fig{decision_bound} where $n = 9$, assuming $\rho= 1/3$ then $n\rho = 3$, the weight combinations are $C_9^{3} * 2^{6} = 5,376$.
Thus the network search space is increased $10.5$ times compared to the full binary network.

\fig{decision_bound}(e) shows the setting of an equivalent ternary network where every weight can take values in $\{-1,0,+1\}$. There are $3^9$ = 19,683 weight combinations, and only 431 unique solutions.
In our model, by using a fixed pruning rate we restrict a fixed number of weights to be 0.
This increases the number of weight combinations and unique solutions, similar to the ternary case.
However, in our case the total number of weight combinations and unique solutions varies with the pruning rate.
\fig{decision_bound}(f) shows that when varying the pruning rate, the maximum number of unique solutions for a pruned network is $\approx 10^3$ making pruned networks similarly powerful as ternary networks, while allowing us to explicitly control the sparsity of the network.

%--------------------------------------------------------------------------
\smallskip \noindent \textbf{Modeling pruning.}
We optimize the pruned sub-networks jointly with the binary connection training.
To create a sub-network, we use a learnable binary mask matrix $\mathbf{M}$ of the same size as $\mathbf{B}$.
Each element ${M}_{ij}$ in $\mathbf{M}$ is 0 when the connection is pruned and 1 otherwise.
The weight connections in the sub-network are given by:
$ \mathbf{C} = \mathbf{M} \odot \mathbf{B}$, where $\odot$ denotes element-wise product.
When searching for the best sub-network, in the forward pass we use $\mathbf{C}$ to compute the loss $\mathcal{L}$, and in the backward pass we compute the  gradient of the loss with respect to $\mathbf{M}$ and $\mathbf{B}$, to update the binary mask and the binary connections. \\

%----------------------------------------------------------------------------------------
\subsection{{Bi-half} Bernoulli regularization}
Our fixed pruning ratio applied to the binary wights, $\mathbf{B}$, may lead to pruning more positive values than negative values, or vice versa.
In information theory~\cite{shulman2004the}, a uniform prior over a binary channel is desirable as it leads to a minimal degradation in channel capacity when compared to the optimal prior.
Thus, a uniform prior is a good initial guess, in the context of deep network compression, where we do not know the optimal prior.
To ensure this, we explicitly model the binary weights as a Bernoulli distribution with a uniform prior.
A Bernoulli distribution describes the probabilities of binary values as $p(-1){=}p_{\mathrm{neg}}$, and $p(+1){=} p_{\mathrm{pos}}$ where $p_{\mathrm{neg}}{+} p_{\mathrm{pos}}{=}1$.
We set the hyperparameter $p_{\mathrm{pos}} {=} p_{\mathrm{neg}} {=} \frac{1}{2}$ under the Bernoulli distribution, which we dub \emph{bi-half}.
The uniform prior over the $-1$ and $+1$ under the Bernoulli distribution, regularizes the problem space: i.e.,  which solutions are preferred.

Going back to the 2$D$ example, in \fig{decision_bound}.(d) the Bernoulli distribution over the weights with equal prior (\emph{bi-half}) regularizes the problem space: it reduces the weight combinations to approximately half, while retaining all unique solutions.
In \fig{decision_bound}(c), we use the same sub-network as in \fig{decision_bound}.(b) yet now with the Bernoulli binary weight distribution.
Here, the \emph{bi-half} regularization reduces the search space $3.6$ times, retaining $90\%$ of the unique decision boundaries compared to \fig{decision_bound}(b).
In \fig{decision_bound}.(f) we see that the \emph{bi-half} regularization reduces the total number of weight combinations consistently for all pruning ratios, while only slightly reducing the unique solutions.

%--------------------------------------------------------------------------------------
\subsection{Optimizing {bi-half} bit distribution and pruning with optimal transport}
\begin{comment}
\begin{figure*}
\centering
\begin{tabular}{cc}
    \includegraphics[width=0.45\textwidth]{pruning.pdf} &
    \includegraphics[width=0.45\textwidth]{ot.pdf} \\
    \scriptsize{(a) Weight combinations vs. pruning ratio.} &
    \scriptsize{(b) Optimal transport.} \\
\end{tabular}
    \caption{
    (a)
    (b) We use optimal transport (OT) to map the distribution of continuous weights $\mathbb{P}_w$ to the distribution of discrete weights $\mathbb{P}_c$ having only 3 possible locations $\{-1,0,1\}$ encoded by $c_j$ (Not to be confused with individual weight values in $\mathbf{C}$.).
    }
    \label{fig:ot}
\end{figure*}
\end{comment}

We jointly optimize the weight values, the weight pruning, and the \emph{bi-half} weight distribution regularization.
To be consistent with previous work, we follow XNOR~\cite{rastegari2016xnor} and apply the optimization per individual filter.
Given a filter flattened to a vector $\mathbf{B} \in \{-1,1\}^D$, then in each forward iteration we mask the weight parameters with probability $\rho$, creating a binary mask $\mathbf{M}\in \{0,1\}^D$.
The weight configuration becomes $\mathbf{C} = \mathbf{M}\odot\mathbf{B}$.
Using the prior \emph{bi-half} distribution, we ensure the binary weights are equally distributed.
When jointly optimizing the mask and the binary weights, we update the discrete matrix $\mathbf{C}$ having three values $\{-1, 0, 1\}$.
Denoting the probability of a $-1, 0$, or $+1$ occurring in $\mathbf{C}$ by $p(c)$, we have for a given pruning ratio $\rho$:
\begin{equation}
    p(c{=}{-1}) {=} \frac{1-\rho}{2}, \  \ p(c{=}0) {=} \rho,  \  \   p(c{=}{+1}) {=} \frac{1-\rho}{2}.
    \label{eq:three1}
\end{equation}

\smallskip\noindent{\textbf{Optimizing the weights.}}
Because the matrix $\mathbf{C}$ is discrete,  we follow~\cite{courbariaux2015binaryconnect,rastegari2016xnor} by using real-value weights $\mathbf{W}$ to aid the training of discrete values, where each binary weight in $\mathbf{C}$ has an associated real-valued weight in $\mathbf{W}$.
In the forward pass we quantize the real-valued weights $\mathbf{W}$ to estimate the matrix $\mathbf{C}$.
Then, we use the estimated matrix $\mathbf{C}$ to compute the loss, and in the backward pass we update the associated real-valued weights $\mathbf{W}$.

\smallskip\noindent\textbf{Optimizing the \emph{bi-half} regularization.}
We define the associated real-valued weights for the filter as $\mathbf{W} \in \mathbb{R}^D$.
We regularize by aligning the real-valued weight distribution with the prior distribution in \eq{three1} and quantize the real-valued weights $\mathbf{W}$ to $\mathbf{C}$.
The empirical distributions of the real-valued variable $\mathbf{W}$ and the discrete variable $\mathbf{C}$, $\mathbb{P}_w$ and $\mathbb{P}_c$, can be written as:
\begin{equation}
    \mathbb{P}_w = \sum_{i=1}^D p_i \delta_{w_i}, \ \ \  \mathbb{P}_c = \sum_{j=1}^{3} q_j \delta_{c_j},
    \label{rewasserp}
\end{equation}
where $\delta_\mathbf{x}$ is the Dirac function at location $\mathbf{x}$.
The $p_i$ and $q_j$ are the probability mass associated to the corresponding distribution locations $w_i$ and $c_j$, where $\mathbb{P}_c$ has only 3 possible locations in the distribution space $\{-1,0,1\}$. %, as displayed in \fig{ot}.(b).
For our target prior distribution in \eq{three1}, the probability mass $q_1 {=} p(c {=} {+1})$ is equal to the probability mass $q_2 {=} p(c {=} {-1})$ that is $q_1 = q_2 = \frac{1-\rho}{2}$, and the probability mass $q_3 {=} p(c {=} 0) {=} \rho$.

To align $\mathbb{P}_w$ with the prior $\mathbb{P}_c$ we use optimal transport (OT)~\cite{villani2003topics} which minimizes the cost of moving the starting distributions $\mathbb{P}_w$  to the target distribution $\mathbb{P}_c$.
Because $\mathbb{P}_w$ and $\mathbb{P}_c$ are only accessible through a finite set of values, the corresponding optimal transport cost is defined as:
\begin{equation}
    \pi_0= \mathop{\min}_{\pi \in \Pi(\mathbb{P}_w, \mathbb{P}_c)} 	\left \langle \pi, \mathbf{D}\right \rangle_F,
    \label{rewasserp0}
\end{equation}
where $\Pi(\mathbb{P}_w, \mathbb{P}_c)$ is the space of the joint probability with marginals $\mathbb{P}_w$ and $\mathbb{P}_c$, and $\pi$ is the general probabilistic coupling that indicates how much mass is transported to push distribution $\mathbb{P}_w$  towards the distribution $\mathbb{P}_c$.
The $\left \langle ., .\right \rangle_F$ denotes the Frobenius dot product,  and $\mathbf{D} \geq 0$ is the cost function matrix whose element  $\mathbf{D}(w_i, c_j)$ denotes the cost of moving a probability mass from location $w_i$ to location $c_j$ in distribution space.
When the cost is defined as a distance, the OT becomes the Wasserstein distance.
We minimize the 1-Wasserstein distance between $\mathbb{P}_w$ and $\mathbb{P}_c$.
This minimization has an elegant closed-form solution based on simply sorting.
For a continuous-valued weights vector $\mathbf{W} \in \mathbb{R}^D$ and pruning ratio $\rho$, we first sort the elements of $\mathbf{W}$, and then assign the top $\frac{1-\rho}{2}$ ratio of the elements to $+1$, the bottom $\frac{1-\rho}{2}$ portion of the elements to $-1$, and assign the remaining  $\rho$ ratio of the elements to $0$, that is:
\begin{equation}
    \ \ \ \  \mathbf{C}= \mathrm{\pi_0}\ (\mathbf{W}) =
    \begin{cases}
    +1,  & \mathrm{ top \ \frac{1-\rho}{2} \ of \ sorted}\ \mathbf{W}\\
    -1, & \mathrm{ bottom \ \frac{1-\rho}{2} \ of \ sorted}\ \mathbf{W}\\
    0, & \mathrm{otherwise}.
    \end{cases}
    \label{eq:behalf1}
\end{equation}

%--------------------------------------------------------------------------------
\smallskip\noindent \textbf{Backward pass optimization.}
We need no special considerations, and directly follow~\cite{courbariaux2015binaryconnect,rastegari2016xnor} for updating the real valued weights $\mathbf{W}$.
As the discrete weights matrix $\mathbf{C}$ have no continuous derivatives, commonly \cite{qin2020forward,rastegari2016xnor} a proxy derivative is used with the straight-through estimator (STE)~\cite{bengio2013estimating}.
We adopt the STE on our cross entropy loss $\mathcal{L}$, to obtain the gradients with respect to $\mathbf{W}$ as $\frac {\partial \mathcal{L}} {\partial \mathbf{W}} = \frac {\partial \mathcal{L}} {\partial \mathbf{C}}$.

%--------------------------------------------------------------------------------
\smallskip\noindent \textbf{Initialization and scaling factor.}
To circumvent exploding gradients, we initialize the real-valued weights using Kaiming normal~\cite{he2015delving}, and standardize per-filter weights to zero-mean.
Following~\cite{glorot2010understanding,he2015delving}, we initialize one \emph{scaling factor} $\alpha$ per layer for the binary weights to keep the activation variance in the forward pass close to~$1$.
Based on the ReLU variance analysis in~\cite{he2015delving} it holds that $\frac{1}{2} D\cdot Var(\alpha{\mathbf{B}}) = 1$, where $D$ is the number of connections and $\mathbf{B}$ are our binary weights.
$\mathbf{B}$ is regularized to a \emph{bi-half} distribution, thus $Var(\mathbf{B}) = 1$, which gives $\alpha = \sqrt{2/D}$.
For a sub-network with pruning ratio $\rho$, the variance in the forward pass is thus not exactly $1$ and the number of connections changes to $(1-\rho) D$.
Therefore, we rescale the initialization scaling factor $\alpha$ by $\sqrt{1/(1-\rho)}$.

%--------------------------------------------------------------------------------
\begin{comment}
\noindent \textbf{Irregular Matrix Storage.}
Compressed Sparse Row (CSR)[];
Binary index[];
Viterbi Approaches[];
Network Pruning for Low-Rank Binary Index[];
Viterbi-based Pruning for Sparse Matrix with Fixed and High Index Compression Ratio []
Double Viterbi: Weight Encoding for High Compression Ratio and Fast On-Chip Reconstruction for Deep Neural Network[]
Structured Compression by Weight Encryption
for Unstructured Pruning and Quantization(0.28 bits/weight).
\end{comment}



==> method_stuff.tex <==
\section{\Model regularization with optimal transport}
\label{methods}
We aim to define a binary network where the weights $\mathbf{B}$ take binary value $\{1,-1\}^d$. 
The training of binary neural networks is challenging due to the discrete nature of binary weight parameters where gradient-based methods cannot be directly applied. 
Following \cite{rastegari2016xnor}, binary weights are associated with real-valued parameters to aid the training of binary network, $\mathbf{W}\in \mathbb{R}^d$.   

We assume a Bernoulli distribution over the binary weights, describing the probabilities of binary values as $p(-1){=}p_{\mathrm{neg}}$, and $p(+1){=} p_{\mathrm{pos}}$ where $p_{\mathrm{neg}}{+} p_{\mathrm{pos}}{=}1$.
Similar to \cite{qin2020forward}, we set the hyperparameter $p_{\mathrm{pos}} {=} p_{\mathrm{neg}} {=} \frac{1}{2}$ under the Bernoulli distribution. 
However, here we enforce that the ratio of the positive ($p_{\mathrm{pos}}$) and negative weights $p_{\mathrm{pos}}$ is at all times equal using optimal transport. We dub this \model.


%=========================================================================================
\subsection{\Model as regularization}
The uniform prior over the $-1$ and $+1$ under the Bernoulli distribution regularizes the problem space, where only a subset of possible weight combinations are preferred.
We illustrate this intuitively on a 2$D$ example for a simple fully-connected neural network with one input layer, one hidden layer, and one output layer in a two-class classification setting.
We consider a 2$D$ binary input vector $\mathbf{x} = [x_1, x_2]^\intercal$, a $2 \times 2$ binary weight matrix $\mathbf{W}$, and a 2$D$ binary bias vector $\mathbf{b}$ as the hidden layer, followed by a $\tanh$ nonlinear activation, and an output layer composed of a $2 \times 1$ binary weight and a binary bias $c$.
Thus, the output of the network is $\sigma( \mathbf{w}^\intercal \tanh(\mathbf{W}^\intercal \mathbf{x} + \mathbf{b}) + c)$,  where $\sigma$ is a sigmoid nonlinearity.
We group all $9$ parameters as a vector $\mathbf{B}$. 
We enumerate all possible binary weight combinations in $\mathbf{B}$, \ie \ $2^9 = 512$, and plot all decision boundaries that separate the input space into two classes as shown in \fig{decision_bound}(a). All possible 512 binary weights combinations offer only $30$ unique decision boundaries.
In \fig{decision_bound}.(b) the Bernoulli distribution over the weights with equal prior (\model) regularizes the problem space: it reduces the weight combinations to approximately half, while retaining all unique solutions.

\begin{figure}[t]
\centering
\begin{tabular}{cc}
    {(a) Full binary network} &
    {(b) \Model network} \\
    \includegraphics[width=0.23\textwidth]{fig/toy/Onecolor_prune0.pdf} &
    \includegraphics[width=0.23\textwidth]{fig/toy/half_half_Prune_0_figure.pdf} \\
    \scriptsize{Weight combinations: 512.} &
    \scriptsize{Weight combinations: 252.} \\
    \scriptsize{Unique solutions: 30.} &
    \scriptsize{Unique solutions: 30.} \\
    \end{tabular}
    \caption{ \small
    2D example for a 9-parameter fully connected binary network $\sigma( \mathbf{w}^\intercal \tanh(\mathbf{W}^\intercal \mathbf{x} + \mathbf{b}) + c)$,  where $\sigma$ is a sigmoid nonlinearity. Weights are in $\{ -1, 1 \}$ or $0$ when pruned.
    (a) Enumeration of all decision boundaries for 9 binary parameters (512 = $2^9$ combinations).
    (d) Weight combinations and unique solutions when using our \model.
    Using the \model works as a regularization, reducing the search-space while retaining the majority of the solutions.
    \todo{Replace the figure.}
    }
 \label{fig:decision_bound}
\end{figure}

%=========================================================================================
\subsection{Optimal transport \model optimization}


%=========================================================================================
\subsection{Relation to existing optimization trends}

In \tab{optimizations} we compare two existing optimization perspectives, approximation view and  inertia-based view as shown in \tab{optimizations}(a) and \tab{optimizations}(c) to our dynamic threshold perspective as shown in \tab{optimizations}(b).  
% the optimization steps of our dynamic threshold viewpoint as shown in \tab{optimizations}(b) to two existing viewpoints, approximation view and inertia-based view as shown in \tab{optimizations}(a) and \tab{optimizations}(c).  
% we compare three different perspectives of binary network optimization 
% To better understand the optimization for binary neural network, in \tab{optimizations} we compare the optimization steps of our dynamic threshold viewpoint as shown in \tab{optimizations}(b) to two existing viewpoints, approximation view and inertia-based view as shown in \tab{optimizations}(a) and \tab{optimizations}(c).  

The approximation viewpoint mainly focuses on minimizing the quantization error between the binarized weight and the real-valued parameter. The introduced real-valued parameter is treated as  real-valued latent weight to apply  traditional optimization techniques including various optimizers and regularizers.  
The whole training steps are shown in \tab{optimizations}(a). During the forward pass the latent weights is binarized using a sign function to obtain binary weights.  Since the gradient of the sign function is zero almost everywhere,  during backward pass a proxy derivative approximated by straight through estimator (STE) \yq{citations} is used to update the latent weights.  
% $\frac {\partial \mathcal{L}} {\partial \mathbf{W}} = \frac {\partial \mathcal{L}} {\partial \mathbf{B}}$
The approximation view introduces an additional layer with latent weights that makes it harder to reason about the effectiveness of different training techniques  in the context of BNNs. 
Also overemphasizing on improving the approximation between binary weight and latent weight  may lead to cumbersome methods that obscure the training process and hinder deeper understanding. 

%=========================================================================================
%=========================================================================================
%=========================================================================================
%=========================================================================================





% we empirically identify and
% study the effectiveness of the various ad-hoc techniques commonly used in the literature, providing best-practices for efficient training of binary models. We show
% that adapting learning rates using second-moment methods is crucial for the successful use of the STE, and that other optimisers can easily get stuck in local
% minima. Efficient convergence and accuracy of binary models often rely on careful finetuning and various ad-hoc techniques interpret the real-valued latent weights the effect of "latent weight"






% Let $\mathbf{X} = \{ \mathbf{x_i}\}_{i = 1}^N$ denote $N$ training images.
% The images are encoded to $K$ compact binary codes $\mathbf{B}\in \{1,-1\}^{N\times K}$, which also denotes the output of our hash coding layer.
%  $\mathbf{U} \in \mathbb{R}^{N\times K}$ would be
% expressed as the continuous feature representations in the last layer of a standard neural network, \eg,  an encoder, which serves as the input to our hash coding layer.
\begin{table*}
	\centering
	\renewcommand{\arraystretch}{1.2}
	\resizebox{1\linewidth}{!}{
	 \setlength{\tabcolsep}{0.6mm}{
	   	\begin{tabular}{l|l|l|l}
    	\toprule
% 			  	Initialization:			 & \multicolumn{3}{l}{  $w$; optimizer $m$; hyper dsdsdsds 
% }
%  \\
%  			  \midrule	 	
	   &
		 	    % &  \multicolumn{2}{c}{Storage Cost (Mbit)} & & \multicolumn{2}{c}{Accuracy (\%)} \\
			     \textbf{\textcircled{a} Approximation view}  & \textbf{\textcircled{b} Our dynamic threshold view} &  \textbf{\textcircled{c} Inertia-based view of Bop}   \\
			  \midrule	
			  	Initialization:			 &  Latent weight $w$; Optimizer $m$; 
& Binary weight $b$; Threshold $w$, \text{sign}($w$) =  \text{sign}($b$) &  Binary weight $b$; Predefined threshold $\tau$;  
 \\
 &   Hyperparameters \alpha, \phi.
& Momentum $m$; Hyperparameters \alpha, \phi.& Momentum $m$; Hyperparameters \phi.
 \\
 			  \midrule	
	Obtain binary weight $b$:			 &   $b\leftarrow \text{sign}(w)$ &
		  	$
		  	b\leftarrow
-b, \  \text{if} \  |w|< \alpha|g|  \ \text{and}\  \text{sign}(g) =  \text{sign}(b)
 $
&
		  	$
		  	b\leftarrow
-b, \  \text{if} \  \tau< |g|  \ \text{and}\  \text{sign}(g) =  \text{sign}(b)
 $
 \\
Compute gradient of $b$:&
   $g\leftarrow m(\bigtriangledown{\ell(b)}, \phi)$  &   $g\leftarrow m(\bigtriangledown{\ell(b)}, \phi)$  &  $g\leftarrow m(\bigtriangledown{\ell(b)}, \phi)$   \\ 		
	Update real-valued $w$:  &
		   $w\leftarrow  w - \alpha g$  & 		  
		  % $w\leftarrow f(w, g, \alpha) $ 	
		   $w\leftarrow  w - \alpha g$  &
		  \\	
		  \midrule
		  Relations & \multicolumn{3}{c} {

\[
\xymatrix@R+0.1pc@C+6pc{
\textbf{\textcircled{a}} \   \ar[r]<2.8pt>^*{\small	{\text{Treat w as dynamic threshold} }} & \ \textbf{\textcircled{b}} \ \ar[r]<2.8pt>^*{\small	{\text{Fixed threshold} } } \ar[l]<2.8pt>^*{\small	{\text{Treat w as latent weight} } } & \ \textbf{\textcircled{c}} \ar[l]<2.8pt>^*{\small	{\text{Dynamic threshold} } } 
%   \\
%   Z \ar[u]<4pt>^*{\gamma_1} \ar[u]<-4pt>_*{\gamma_2}
%     \ar[ur]_*{e \circ \gamma_1 = e \circ \gamma_2}
}
\]
}
		  % \\
		  % &&
		  \\
	      \bottomrule
		\end{tabular}
	}
	}
% 	\vspace{0.05in}
	\caption{
	\small
% 	\textbf{Exp 2.1: Storage savings for different architectures.}
 Different optimization perspectives . 
}
	\label{tab:optimizations}
	
\end{table*}

%This paper we  offer a new interpretation of existing BNN training algorithms to
%study the effectiveness of the various commonly used training techniques and further provide a novel bi-half binarization method to maximize entropy capacity of binary weight parameters.   
% We will introduce some notations.
%This section we will detailedly introduce the proposed hashing coding layer.
%We will first introduce some notations.
%Let $\mathbf{B}\in \{1,-1\}^d$ denote one binary   weight filter. 
%The training of  binary neural networks is  challenging due to the discrete nature of binary weight parameters where gradient-based methods cannot be directly applied. 
%Usually each binary weight is associated with one real-valued parameter to aid the training of binary network, forming a real-valued parameter matrix  $\mathbf{W}\in \mathbb{R}^d$.   

\subsection{Binary Neural Network  Optimization}
In \tab{optimizations} we compare two existing optimization perspectives, approximation view and  inertia-based view as shown in \tab{optimizations}(a) and \tab{optimizations}(c) to our dynamic threshold perspective as shown in \tab{optimizations}(b).  
% the optimization steps of our dynamic threshold viewpoint as shown in \tab{optimizations}(b) to two existing viewpoints, approximation view and inertia-based view as shown in \tab{optimizations}(a) and \tab{optimizations}(c).  
% we compare three different perspectives of binary network optimization 
% To better understand the optimization for binary neural network, in \tab{optimizations} we compare the optimization steps of our dynamic threshold viewpoint as shown in \tab{optimizations}(b) to two existing viewpoints, approximation view and inertia-based view as shown in \tab{optimizations}(a) and \tab{optimizations}(c).  

The approximation viewpoint mainly focuses on minimizing the quantization error between the binarized weight and the real-valued parameter. The introduced real-valued parameter is treated as  real-valued latent weight to apply  traditional optimization techniques including various optimizers and regularizers.  
The whole training steps are shown in \tab{optimizations}(a). During the forward pass the latent weights is binarized using a sign function to obtain binary weights.  Since the gradient of the sign function is zero almost everywhere,  during backward pass a proxy derivative approximated by straight through estimator (STE) \yq{citations} is used to update the latent weights.  
% $\frac {\partial \mathcal{L}} {\partial \mathbf{W}} = \frac {\partial \mathcal{L}} {\partial \mathbf{B}}$
The approximation view introduces an additional layer with latent weights that makes it harder to reason about the effectiveness of different training techniques  in the context of BNNs. 
Also overemphasizing on improving the approximation between binary weight and latent weight  may lead to cumbersome methods that obscure the training process and hinder deeper understanding. 


% Many training tricks\yq{citations} have been proposed to  improve the approximation and achieve
% impressive results. 
% The approximation perspective still remains unclear including


% which is to see the
% binary weights as an approximation to the real-valued weight vector


% Currently many existing works \yq{citations} introduce the real-valued latent weights to accumulate small update steps  and during training  the quantization error between the latent weight and the quantized binary weight is minimized.
% The binary weight is treated as an approximation to the latent weight. The optimization steps are shown in  \tab{optimizations}(a). During the forward pass the latent weights is binarized using a sign function to obtain binary weights.  Since the gradient of the sign function is zero almost everywhere,  during backward pass a proxy derivative approximated by straight through estimator (STE) \yq{citations} is used to update the latent weights.  
% Many training tricks\yq{citations} have been proposed to  improve the approximation and achieve
% impressive results. 
% The approximation perspective still remains unclear including
% i) s


% Under approximation point of view, many training  tricks\yq{citations}  have been proposed to reduce  quantization error. For example new regularization terms\yq{citations} are proposed to encourage latent weights to be bipolar. 
% With the introduced latent weight, many insights and intuitions inspired by real-valued networks are directly translated to BNNs including various optimizers and regularizers.  
% It still remains unclear from the approximation viewpoint, such as the effect of regularization term, weight clipping and learning rate. 
% The approximation-view based methods  work well in practice but the reasons behind its effectiveness are unknown.



% For example, 
% the controversy of the added regularization term is an imposed L2 regularization on latent weight helpful

% Thirdly, we reveal that instead of imposing L2 regularization,
% driving all weights to zero which contradicts with the setting
% of BinaryNets, we introduce a regularization term that encourages the weights to be bipolar
% even for the 

% A better understanding of latent
% weights will aid the deployment of existing optimization techniques and can guide the development
% of novel methods.




Recently \yq{citations} proposed a new method that challenges the view of approximation. 
They argue that the approximation viewpoint is problematic and the latent weights should not be treated as weights at all.
Instead, they explain latent real-valued weights as encoding inertia against binary weight flip.
Based on this perspective, they propose  
a latent-free binary optimizer (Bop) as shown in  \tab{optimizations}(c) which looks at an exponential moving average of gradients during training and determine whether to flip each weight by comparing the moving average with a fixed threshold. 
The Bop method is conceptually simpler than current methods  \yq{citations}  but in practice this optimization does not perform very well which is sensitive to the selection of the predefined threshold. Critically the Bop method is difficult to incorporate the commonly used techniques such as regularizers and learning rate decay.   

In \tab{optimizations}(b), we  explain the real-valued latent weight as  the dynamic threshold.
The additional sign layer is interpreted in terms of binary weight flips.
Specifically, the dynamic threshold $w$ is compared with the scaled moving average gradients $\alpha g$  as in \fig{envenflip}(a) to decide whether to flip each binary weight $b$,
%  \begin{equation}
% b_t=
% \begin{cases}
% -b_{t-1}, & \text{if} \  |w_{t-1}|< \alpha|g_t|  \ \text{and}\  \text{sign}(g_t) =  \text{sign}(b_{t-1})\\
% b_{t-1}, & \mathrm{otherwise}.
% \end{cases}
% \label{behalf}
% \end{equation}
 \begin{equation}
 b = 
\begin{cases}
\ {-b}, & \text{if} \  |w|< \alpha|g|  \ \text{and}\  \text{sign}(g) =  \text{sign}(b)\\
\ {b}, & \mathrm{otherwise}
\end{cases}
\label{eq:behalf},
\end{equation}
where $\alpha$ is a scaling variable much like learning rate.
As compared to existing Bop method \yq{citation}, the difference is that instead of using a fixed threshold $\tau$ in \tab{optimizations}(c), we introduce a dynamic threshold which is updated with a heuristic way  $w = w - \alpha g$ where $g$ is a pseudo-gradient. 
We study some commonly
used techniques such as  weight clipping, regularization and learning rate decay, and show that some of these techniques are not crucial in training well-performing BNNs.
% We further study the effectiveness of the various commonly  used  training  techniques.
\begin{itemize}
\item $L_2$ regularization. We find that applying L2-regularization to the real-valued threshold  should not lead to any regularization. It only  affects binary weight flips by controlling the magnitude of threshold as shown in \fig{envenflip}(a). 
\item Bipolar regularization.
Some recent works \yq{citation}
%How to Train a Compact Bnn, 1-Bit CNNs, Rotated Binary Neural Network, BNN++
introduce regularization term or design specific loss function to encourage real-valued parameter to  binary weight. We show that encouraging  real-valued threshold to be bipolar distribution is not necessary. 
\item Weight clipping. 
Clipping is used to restrict the latent weights as in common view between a region that avoids latent weights grow very large. We reveal that clipping of the threshold is not crucial during training. 
% \item Scaling factors. 
% add a real-valued scaling factor to imporve the 
\item Learning rate decay.  
Bop claims that scaling of the learning rate does not affect training.  
We find that varying  learning rate as  in \eq{behalf} will affect binary weight flips.
Gradually reducing learning rate will decrease weight flips. 
We also find that the learning rate decay and the $L_2$ regularization are indispensable to each other.
% This variable $\alpha$ should 
% As in real-valued network, learning rate is used to control the updated step size 
\end{itemize}
Our interpretation of latent weights as dynamic threshold is easy to reason about the effectiveness of various optimization techniques.  
We will further explore their effectiveness  in the experiments section. 
% according to some rules $f$ as: 
% \begin{equation}
% w_{t} = f(w_{t-1}, g_t, \alpha).
% \label{eq:updatethreshold}
% \end{equation}

% We elaborate the relationship between different views: \textit{i)}  By setting the threshold in \eq{updatethreshold} as a constant value  $f(w_{t-1}, g_t, \alpha) = \tau$, our perspective degrades into Bop; \textit{ii)} If the threshold in \eq{updatethreshold} is pushed in the negative direction of a pseudo-gradient $g_t$ as  $f(w_{t-1}, g_t, \alpha) = w_{t-1} - \alpha g_t$, our perspective can be seen as the common  approximation viewpoint.  We further study the effectiveness of the various commonly  used  training  techniques.

% \begin{itemize}
% %\vspace{-2mm}	

\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{fig/eweight_hitting/weight_gradhitting.png} \\ 
    \small {(a) Flipping by comparing dynamic threshold with gradient}  \\ 
        \includegraphics[width=0.47\textwidth]{fig/eweight_hitting/flipped_uneven.png}\\
    \small {(b)  Sign  has  unevenly  flipping within binary weight filter}  \\         
        \includegraphics[width=0.47\textwidth]{fig/eweight_hitting/bihalf_flipped_even.png}
            \small {(c) Bi-half    has  evenly  flipping within binary weight filter.}  \\ 
    \caption{\small
    Binary weight flips during training. (a) single binary weight flip; (b, c):  binary weight flips within a filter
    % \textbf{Exp 2: Which bit-ratio is preferred?}
    % On CIFAR-10/100 for Conv2 we vary the probabilities of binary values.
    % The x-axis shows the prior probability of a positive binary value (\eg +1), which is the hyperparameter $p_{pos}$ of the Bernoulli distribution.
    % The y-axis denotes the pruning ratio $\rho$.
    % The color bar indicates the distribution of values for the top-1 accuracy, where dark red is 100\% and dark blue is 0\%.
    % By varying the probability of pruned weights, the best performance is consistently obtained along the \emph{bi-half} solid line.
    }
    \label{fig:envenflip}
\end{figure}

% \item  The first is
% the controversy of using regularization.  Some previous works \yq{citation} claim that imposing a $L_2$ regularization is contradictory to the BNN setting, instead they introduce a regularization term to encourage real-valued parameter to approximate binary weight  as 1 or -1. 
% %\vspace{-2mm}

% \item 

% \end{itemize}

\begin{comment}
f imposing L2 regularization,
driving all weights to zero which contradicts with the setting
of BinaryNets, we introduce a regularization term that encourages the weights to be bipolar.
As we have argued, it is not clear that applying L2-regularization or weight decay
to the latent weights should lead to any regularization at all. 

\end{comment}


%---------------------------------------------------------------------------------
%---------------------------------------------------------------------------------
%---------------------------------------------------------------------------------
\subsection{Half-half solution space}

1. Sign: decide whether to flip each binary weight independently. As shown in \fig{envenflip}(b), sign has unevenly flipping within a binary weight filter.  

2. IR-net: Balance the threshold with subtracting their mean within a filter to maximize entropy capacity of  binary weight parameters 

3. 
We  precisely control the binary weight distribution such that the -1 and +1 symbols are equally distributed at all times during training: a half-half distribution.
To maximize entropy capacity of binary weight parameters


\todo{In the google doc we said we would keep here the visualization for the solution space reduction for half-half}

%---------------------------------------------------------------------------------
%---------------------------------------------------------------------------------
%---------------------------------------------------------------------------------

% We  offer a new interpretation of existing BNN training algorithms which explains real-valued latent  weight as adaptive threshold 
% interprets the latent weights as inertia

%  and further provide a novel bi-half binarization method to maximize entropy capacity of binary weight parameters.   
% We interpret the latent weights as inertia differs 
% This optimization is simple and requires less memory during training. 
% The proposed Bop interprets BNN optimization in terms of weight flips.  
% which enables a better understanding of different training techniques. 
% The selection of the threshold is a difficult choice in the algorithm. As a result it can be seen that BoP effectively reduces the number of variables to be optimized to two.




% Hyperparameter schedules could also target the threshold, τ , (or an adaptive variation of τ ). We
% hypothesize one should select for strong signals (i.e. high τ ) in the first stages of training, and make
% training more sensitive by lowering τ over time, perhaps while simultaneously lowering γ. However,
% we stress once again that such intuitions may prove unreliable in this unexplored context.


% A larger threshold, means more confident to encode this binary weights to 1 
% grows, a stronger gradient-signal is required to make the corresponding binary weight flip. 




% [Back to Simplicity, BOP, BNN++, Real-to-bin, How adam..
% ]


% Recently Helwegen et al. (2019) proposed a new method
% that goes against the justification behind STE. They argue that “latent” weights used in STE based methods do not exist.




% cooperate with traditional optimization techniques inspired by real-valued networks such as optimizers and regularizers, 
% Momentum, Adam, weight decay, are  
% are difficult to translate to BNNs
\begin{comment}
1. our perspective: carefully weight decay is good, STE opposite 
Q:
A:

BOP problem: why apply reg and lr to Inertia? 


S: BNN is important, storage-computational 

C: 



Together, the redefinition of latent weights as inertia and the introduction
of Bop enable a better understanding of BNN optimization and open up the way
for further improvements in training methodologies for BNNs

\end{comment}


% \begin{table*}
% 	\centering
% 	\renewcommand{\arraystretch}{1.2}
% 	\resizebox{1\linewidth}{!}{
% % 	 \setlength{\tabcolsep}{0.95mm}{
% 	   	\begin{tabular}{|l|l|l|}
%      \hline	
		 	   
% 		 	    % &  \multicolumn{2}{c}{Storage Cost (Mbit)} & & \multicolumn{2}{c}{Accuracy (\%)} \\
% 			     \textbf{Approximation view with STE}  & \textbf{Proposed dynamic threshold view} &  \textbf{Inertia-based view of Bop}   \\
% 			    \hline	
% 		  Binarize latent weight: $b_{t}\leftarrow \text{sign}(w_t)$ & 
% 		  	\multirow{2}*{$
% b_{t+1} =
% \begin{cases}
% -b_{t},  & \text{if} \ |g_{t}| > \tau \ \text{and}\  \text{sign}(g_{t}) = \text{sign}({b_{t})} \\
%  \ \ \ b_{t}, & \mathrm{otherwise}
% \end{cases} $}
% &  
% 	\multirow{2}*{$
% b_{t+1} =
% \begin{cases}
% -b_{t},  & \text{if} \ |g_{t}| > \tau \ \text{and}\  \text{sign}(g_{t}) = \text{sign}({b_{t})} \\
%  \ \ \ b_{t}, & \mathrm{otherwise}
% \end{cases} $}
%  \\
% 		  Gradient of $b_t$:   $g_{t}\leftarrow m_t(\bigtriangledown{\ell(b_t)}, \phi)$  &  &   \\ 		
% 		  Update: $w_{t+1}\leftarrow w_{t} - \alpha_t g_t$  &  &  
		  
% 		  \\	
% 			 %   MobileNet~\cite{howard2017mobilenets}       & 105.90  & 0.76 &  65.66$\pm$ 0.09 &45.36$\pm$3.24  \\
% 		  %      ShuffleNet~\cite{zhang2018shufflenet}      & 33.34   & 0.32 &  71.78$\pm$ 0.28  &  60.25$\pm$0.63  \\
% 	     \hline	
% 		\end{tabular}
% % 	}
% 	}
% % 	\vspace{0.05in}
% 	\caption{
% 	\small
% % 	\textbf{Exp 2.1: Storage savings for different architectures.}
% 	 Accuracy comparison over different methods by training the Conv2/4/6/8 networks on Cifar-10.
% }
% 	\label{tab:optimization}
	
% \end{table*}


% \begin{table*}
% 	\centering
% 	\renewcommand{\arraystretch}{1.2}
% 	\resizebox{1\linewidth}{!}{
% % 	 \setlength{\tabcolsep}{0.95mm}{
% 	   	\begin{tabular}{|l|l|l|}
%      \hline	
		 	   
% 		 	    % &  \multicolumn{2}{c}{Storage Cost (Mbit)} & & \multicolumn{2}{c}{Accuracy (\%)} \\
% 			     \textbf{Approximation view with STE}  & \textbf{Proposed dynamic threshold view} &  \textbf{Inertia-based view of Bop}   \\
% 			    \hline	
% 		  Binarization: $b_{i}\leftarrow \text{sign}(w_i)$ & 
% 		  	$
% 		  	b_{i}\leftarrow 
% -b_{i}; \  \text{if} \  |w_i|< |g_{i}|  \ \text{and}\  \text{sign}(g_{i}) =  \text{sign}(b_{i})
%  $
% &  
% 		  	$
% 		  	b_{i}\leftarrow 
% -b_{i}; \  \text{if} \  \tau< |g_{i}|  \ \text{and}\  \text{sign}(g_{i}) =  \text{sign}(b_{i})
%  $
%  \\
% 		  Gradient:   $g_{i}\leftarrow m(\bigtriangledown{\ell(b_i)}, \phi)$  &  Gradient:   $g_{i}\leftarrow m(\bigtriangledown{\ell(b_i)}, \phi)$  & Gradient:   $g_{i}\leftarrow m(\bigtriangledown{\ell(b_i)}, \phi)$   \\ 		
% 		  Update: $w_{i}\leftarrow w_{i} - \alpha g_i$  & 		  Update: $w_{i}\leftarrow w_{i} - \alpha g_i$ 		  &   
		  
% 		  \\	
% 			 %   MobileNet~\cite{howard2017mobilenets}       & 105.90  & 0.76 &  65.66$\pm$ 0.09 &45.36$\pm$3.24  \\
% 		  %      ShuffleNet~\cite{zhang2018shufflenet}      & 33.34   & 0.32 &  71.78$\pm$ 0.28  &  60.25$\pm$0.63  \\
% 	     \hline	
% 		\end{tabular}
% % 	}
% 	}
% % 	\vspace{0.05in}
% 	\caption{
% 	\small
% % 	\textbf{Exp 2.1: Storage savings for different architectures.}
% 	 Accuracy comparison over different methods by training the Conv2/4/6/8 networks on Cifar-10.
% }
% 	\label{tab:optimization}
	
% \end{table*}


% \begin{table*}
% 	\centering
% 	\renewcommand{\arraystretch}{1.2}
% 	\resizebox{1\linewidth}{!}{
% 	 \setlength{\tabcolsep}{0.85mm}{
% 	   	\begin{tabular}{l|l|l|l}
%     	\toprule
% 	   &
% 		 	    % &  \multicolumn{2}{c}{Storage Cost (Mbit)} & & \multicolumn{2}{c}{Accuracy (\%)} \\
% 			     \textbf{Approximation view with STE}  & \textbf{Proposed dynamic threshold view} &  \textbf{Inertia-based view of Bop}   \\
% 			  \midrule		
% 	Update $b_i$:			 &   $b_{i}\leftarrow \text{sign}(w_i)$ & 
% 		  	$
% 		  	b_{i}\leftarrow 
% -b_{i}; \  \text{if} \  |w_i|< |g_{i}|  \ \text{and}\  \text{sign}(g_{i}) =  \text{sign}(b_{i})
%  $
% &  
% 		  	$
% 		  	b_{i}\leftarrow 
% -b_{i}; \  \text{if} \  \tau< |g_{i}|  \ \text{and}\  \text{sign}(g_{i}) =  \text{sign}(b_{i})
%  $
%  \\
%  Gradient:&
%   $g_{i}\leftarrow m(\bigtriangledown{\ell(b_i)}, \phi)$  &   $g_{i}\leftarrow m(\bigtriangledown{\ell(b_i)}, \phi)$  &  $g_{i}\leftarrow m(\bigtriangledown{\ell(b_i)}, \phi)$   \\ 		
% 	Update $w_i$:  &
% 		   $w_{i}\leftarrow w_{i} - \alpha g_i$  & 		  $w_{i}\leftarrow w_{i} - \alpha g_i$ 		  &   
		  
% 		  \\	
% 			 %   MobileNet~\cite{howard2017mobilenets}       & 105.90  & 0.76 &  65.66$\pm$ 0.09 &45.36$\pm$3.24  \\
% 		  %      ShuffleNet~\cite{zhang2018shufflenet}      & 33.34   & 0.32 &  71.78$\pm$ 0.28  &  60.25$\pm$0.63  \\
% 	      \bottomrule
% 		\end{tabular}
% 	}
% 	}
% % 	\vspace{0.05in}
% 	\caption{
% 	\small
% % 	\textbf{Exp 2.1: Storage savings for different architectures.}
% 	 Accuracy comparison over different methods by training the Conv2/4/6/8 networks on Cifar-10.
% }
% 	\label{tab:optimization}
	
% \end{table*}














% \noindent \textbf{Approximation.}
% However, due to the binarization function modifications do
% not alter the behavior of the network unless a sign change occurs

% Optimization of Binarized Neural Networks (BNNs) currently relies on real-valued
% latent weights to accumulate small update steps. In this paper, we argue that these
% latent weights cannot be treated analogously to weights in real-valued networks.

% \noindent \textbf{Ours.}
% BOP: In the optimization procedure defined by Algorithm 1, scaling of the learning rate does not have the role one may expect, as is made clear by the following theorem:



% The concept of inertia enables us to better understand what happens during the optimization of BNNs.
% Below we review some key aspects of the optimization procedure from the perspective of inertia.

